Spectral approximation of aperiodic Schr\"odinger operators

We study the (H\"older-)continuous behavior of the spectra belonging to a family of linear bounded operators $(A_t)_{t\in T}$ indexed by a topological space $T$. For the cases of self-adjoint, unitary and normal operators, a characterization of the continuity of $\Sigma:T\to \mathcal{K}(\mathbb{R}), t\mapsto \sigma(A_t),$ is proven while the distance of the spectra is measured by the Hausorff metric. If $T$ is a metric space, the H\"older-continuous behavior of $\Sigma$ is characterized for self-adjoint and unitary operators. Here we observe interesting effects, namely the rate of convergence is bisect whenever spectral gaps closes. Based on this, we provide a tool to prove the continuity of the spectra for large classes of operators. In particular, we apply this theory to generalized Schr\"odinger operators and show that the continuity of the spectra is characterized by the continuous variation of the underlying dynamical systems. Finally, we analyze the existence of periodic dynamical systems approximating a given dynamical system. This leads to periodic approximations of the corresponding Schr\"odinger operators by the previously developed theory. We prove that local symmetries of the patterns and the presence of a substitution is a sufficient criteria for periodic approximations of subshifts in $\mathbb{Z}^d$. For $d=1$, a characterization is proven for the existence of periodic approximations. For these approaches, the notion of a dictionary is further developed and defined independently of a given configuration. We prove that the set of dictionaries equipped with the local pattern topology is homeomorphic to the space of subshifts. This yields a useful tool to analyze these systems. Furthermore, it delivers the connection of the existence of periodic orbits in a subshift of finite type and the existence of periodic approximations for subshifts.

==> references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%								   	%
%				Paper			   	%
%								   	%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article {Ana79,
    AUTHOR = {Anantharaman-Delaroche, C.},
     TITLE = {Action moyennable d'un groupe localement compact sur une
              alg\`ebre de von {N}eumann},
   JOURNAL = {Math. Scand.},
  FJOURNAL = {Mathematica Scandinavica},
    VOLUME = {45},
      YEAR = {1979},
    NUMBER = {2},
     PAGES = {289--304},
      ISSN = {0025-5521},
     CODEN = {MTSCAN},
   MRCLASS = {22D25 (46L10)},
  MRNUMBER = {580607 (82f:22006)},
MRREVIEWER = {Pierre Eymard},
}

@article {Ana87,
    AUTHOR = {Anantharaman-Delaroche, C.},
     TITLE = {Syst\`{e}mes dynamiques non commutatifs et moyennabilit\'{e}},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {279},
      YEAR = {1987},
    NUMBER = {2},
     PAGES = {297--315},
      ISSN = {0025-5831},
     CODEN = {MAANA},
   MRCLASS = {46L55 (22D25 22D40 43A07 43A35)},
  MRNUMBER = {919508 (89f:46127)},
MRREVIEWER = {Elliot C. Gootman},
       DOI = {10.1007/BF01461725},
       URL = {http://dx.doi.org/10.1007/BF01461725},
}

@incollection {AnRe01,
    AUTHOR = {Anantharaman, C. and Renault, J.},
     TITLE = {Amenable groupoids},
 BOOKTITLE = {Groupoids in analysis, geometry, and physics ({B}oulder, {CO},
              1999)},
    SERIES = {Contemp. Math.},
    VOLUME = {282},
     PAGES = {35--46},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2001},
   MRCLASS = {46L55 (22A22 22D25 58H05)},
  MRNUMBER = {1855241 (2002g:46110)},
       DOI = {10.1090/conm/282/04677},
       URL = {http://dx.doi.org/10.1090/conm/282/04677},
}

@article {And58,
  title = {Absence of Diffusion in Certain Random Lattices},
  author = {Anderson, P. W.},
  journal = {Phys. Rev.},
  volume = {109},
  issue = {5},
  pages = {1492--1505},
  numpages = {0},
  year = {1958},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.109.1492},
  url = {http://link.aps.org/doi/10.1103/PhysRev.109.1492}
}


@misc {Ana16,
    AUTHOR = {Anantharaman-Delaroche, C.},
     TITLE = {Some remarks about the weak containment property for groupoids and semigroups},
      NOTE = {arXiv:1604.01724},
      YEAR = {2016},
       URL = {http://arxiv.org/abs/1604.01724},
}

@article {AnPu98,
    AUTHOR = {Anderson, J. E. and Putnam, I. F.},
     TITLE = {Topological invariants for substitution tilings and their
              associated {${C}^{\ast}$}-algebras},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {18},
      YEAR = {1998},
    NUMBER = {3},
     PAGES = {509--537},
      ISSN = {0143-3857},
   MRCLASS = {46L55 (19K99 37B50 54H20)},
  MRNUMBER = {1631708 (2000a:46112)},
MRREVIEWER = {G. A. Noskov},
       DOI = {10.1017/S0143385798100457},
       URL = {http://dx.doi.org/10.1017/S0143385798100457},
}

@preamble{
   "\def\cprime{$'$} "
}
@article {Arn61,
    AUTHOR = {Arnol{\cprime}d, V. I.},
     TITLE = {Small denominators. {I}. {M}apping the circle onto itself},
   JOURNAL = {Izv. Akad. Nauk SSSR Ser. Mat.},
  FJOURNAL = {Izvestiya Akademii Nauk SSSR. Seriya Matematicheskaya},
    VOLUME = {25},
      YEAR = {1961},
     PAGES = {21--86},
      ISSN = {0373-2436},
   MRCLASS = {32.44 (57.48)},
  MRNUMBER = {0140699},
MRREVIEWER = {J. Moser},
}

@article {Arn62,
    AUTHOR = {Arnol{\cprime}d, V. I.},
     TITLE = {On the classical perturbation theory and the stability problem
              of planetary systems},
   JOURNAL = {Dokl. Akad. Nauk SSSR},
  FJOURNAL = {Doklady Akademii Nauk SSSR},
    VOLUME = {145},
      YEAR = {1962},
     PAGES = {487--490},
      ISSN = {0002-3264},
   MRCLASS = {85.57 (57.48)},
  MRNUMBER = {0142388},
MRREVIEWER = {E. Leimanis},
}

@article {AvBoDa12,
    AUTHOR = {Avila, A. and Bochi, J. and Damanik, D.},
     TITLE = {Opening gaps in the spectrum of strictly ergodic
              {S}chr\"odinger operators},
   JOURNAL = {J. Eur. Math. Soc. (JEMS)},
  FJOURNAL = {Journal of the European Mathematical Society (JEMS)},
    VOLUME = {14},
      YEAR = {2012},
    NUMBER = {1},
     PAGES = {61--106},
      ISSN = {1435-9855},
   MRCLASS = {37A20 (37A25 39A70 47B36)},
  MRNUMBER = {2862034},
MRREVIEWER = {Helge Kr{\"u}ger},
       DOI = {10.4171/JEMS/296},
       URL = {http://dx.doi.org/10.4171/JEMS/296},
}

@article {AvSi81,
    AUTHOR = {Avron, J. and Simon, B.},
     TITLE = {Almost periodic {S}chr\"odinger operators. {I}. {L}imit
              periodic potentials},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {82},
      YEAR = {1981/82},
    NUMBER = {1},
     PAGES = {101--120},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {34B25 (35P05 47E05)},
  MRNUMBER = {638515 (84i:34023)},
       URL = {http://projecteuclid.org/euclid.cmp/1103920456},
}

@article {AvSi83,
    AUTHOR = {Avron, J. and Simon, B.},
     TITLE = {Almost periodic {S}chr\"odinger operators. {II}. {T}he
              integrated density of states},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {50},
      YEAR = {1983},
    NUMBER = {1},
     PAGES = {369--391},
      ISSN = {0012-7094},
     CODEN = {DUMJAO},
   MRCLASS = {34B25 (35P05 81C10)},
  MRNUMBER = {700145 (85i:34009a)},
MRREVIEWER = {W. O. Amrein},
       DOI = {10.1215/S0012-7094-83-05016-0},
       URL = {http://dx.doi.org/10.1215/S0012-7094-83-05016-0},
}

@article {AvSi85,
    AUTHOR = {Avron, J. and Simon, B.},
     TITLE = {Stability of gaps for periodic potentials under variation of a
              magnetic field},
   JOURNAL = {J. Phys. A},
  FJOURNAL = {Journal of Physics. A. Mathematical and General},
    VOLUME = {18},
      YEAR = {1985},
    NUMBER = {12},
     PAGES = {2199--2205},
      ISSN = {0305-4470},
     CODEN = {JPHAC5},
   MRCLASS = {81C12 (35R99)},
  MRNUMBER = {804317 (87e:81039)},
MRREVIEWER = {Lawrence E. Thomas},
       URL = {http://stacks.iop.org/0305-4470/18/2199},
}

@article {AvMoSi91,
    AUTHOR = {Avron, J. E. and van Mouche, P. and Simon, B.},
     TITLE = {Erratum: ``{O}n the measure of the spectrum for the almost
              {M}athieu operator''},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {139},
      YEAR = {1991},
    NUMBER = {1},
     PAGES = {215},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {39A70 (39A12 47B39 47N50 82B05)},
  MRNUMBER = {1116417 (92d:39014b)},
       URL = {http://projecteuclid.org/euclid.cmp/1104203143},
}

@incollection{Baa02,
   author = {Baake, M.},
    title = {A Guide to Mathematical Quasicrystals},
booktitle = {Quasicrystals: An Introduction to Structure, Physical Properties and Applications},
     year = {2002},
publisher = {Springer Berlin Heidelberg},
  address = {Berlin, Heidelberg},
    pages = {17--48},
     isbn = {978-3-662-05028-6},
      doi = {10.1007/978-3-662-05028-6_2},
      url = {http://dx.doi.org/10.1007/978-3-662-05028-6_2},
}

@article {BaLe04,
    AUTHOR = {Baake, M. and Lenz, D.},
     TITLE = {Dynamical systems on translation bounded measures: pure point
              dynamical and diffraction spectra},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {24},
      YEAR = {2004},
    NUMBER = {6},
     PAGES = {1867--1893},
      ISSN = {0143-3857},
   MRCLASS = {37A15 (22D40 37N20)},
  MRNUMBER = {2106769},
MRREVIEWER = {Manfred Einsiedler},
       DOI = {10.1017/S0143385704000318},
       URL = {http://dx.doi.org/10.1017/S0143385704000318},
}

@article {BaLeMo07,
    AUTHOR = {Baake, M. and Lenz, D. and Moody, R. V.},
     TITLE = {Characterization of model sets by dynamical systems},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {27},
      YEAR = {2007},
    NUMBER = {2},
     PAGES = {341--382},
      ISSN = {0143-3857},
   MRCLASS = {37A15 (37B99 52C23)},
  MRNUMBER = {2308136},
MRREVIEWER = {Teturo Kamae},
       DOI = {10.1017/S0143385706000800},
       URL = {http://dx.doi.org/10.1017/S0143385706000800},
}

@article {BaGaeGr13,
    AUTHOR = {Baake, M. and G{\"a}hler, F. and Grimm, U.},
     TITLE = {Examples of substitution systems and their factors},
   JOURNAL = {J. Integer Seq.},
  FJOURNAL = {Journal of Integer Sequences},
    VOLUME = {16},
      YEAR = {2013},
    NUMBER = {2},
     PAGES = {Article 13.2.14, 18},
      ISSN = {1530-7638},
   MRCLASS = {37B10 (52C22)},
  MRNUMBER = {3032397},
MRREVIEWER = {Karsten Keller},
}

@misc {BaDaGr15,
    AUTHOR = {Baake, M. and Damanik, D. and Grimm, U.},
     TITLE = {What is Aperiodic Order?},
      NOTE = {arXiv:1512.05104},
      YEAR = {2015},
       URL = {http://arxiv.org/abs/1512.05104},
}

@article {BaBeRa90,
     AUTHOR = {Barelli, A. and Bellissard, J. and Rammal, R.},
     TITLE = {Spectrum of {$2$}{D} {B}loch electrons in a periodic magnetic
              field: algebraic approach},
   JOURNAL = {J. Physique},
  FJOURNAL = {Le Journal de Physique},
    VOLUME = {51},
      YEAR = {1990},
    NUMBER = {19},
     PAGES = {2167--2185},
      ISSN = {0302-0738},
     CODEN = {JOPQAG},
   MRCLASS = {82D55 (81V70)},
  MRNUMBER = {1156191},
}

@article {Bee93,
    AUTHOR = {Beer, G.},
     TITLE = {On the {F}ell topology},
   JOURNAL = {Set-Valued Anal.},
  FJOURNAL = {Set-Valued Analysis. An International Journal Devoted to the
              Theory of Multifunctions and its Applications},
    VOLUME = {1},
      YEAR = {1993},
    NUMBER = {1},
     PAGES = {69--80},
      ISSN = {0927-6947},
     CODEN = {SVANEG},
   MRCLASS = {54B20 (49J45)},
  MRNUMBER = {1230370 (95a:54024)},
       DOI = {10.1007/BF01039292},
       URL = {http://dx.doi.org/10.1007/BF01039292},
}

@article {BLT83,
    AUTHOR = {Bellissard, J. and Lima, R. and Testard, D.},
     TITLE = {A metal-insulator transition for the almost {M}athieu model},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {88},
      YEAR = {1983},
    NUMBER = {2},
     PAGES = {207--234},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {82A57 (39B10 47B39 81C10 82A65)},
  MRNUMBER = {696805},
MRREVIEWER = {W. Kirsch},
       URL = {http://projecteuclid.org/euclid.cmp/1103922281},
}

@incollection {Bel85,
    AUTHOR = {Bellissard, J.},
     TITLE = {Stability and instability in quantum mechanics},
 BOOKTITLE = {Schr\"odinger operators ({C}omo, 1984)},
    SERIES = {Lecture Notes in Math.},
    VOLUME = {1159},
     PAGES = {204--229},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1985},
   MRCLASS = {81C10 (58F27)},
  MRNUMBER = {824989},
MRREVIEWER = {Helmut R{\"u}ssmann},
       DOI = {10.1007/BFb0080334},
       URL = {http://dx.doi.org/10.1007/BFb0080334},
}

@incollection {Bel86,
    AUTHOR = {Bellissard, J.},
     TITLE = {{$K$}-theory of {$C^\ast$}-algebras in solid state physics},
 BOOKTITLE = {Statistical mechanics and field theory: mathematical aspects
              ({G}roningen, 1985)},
    SERIES = {Lecture Notes in Phys.},
    VOLUME = {257},
     PAGES = {99--156},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1986},
   MRCLASS = {46L60 (19K56 46L80 82A15)},
  MRNUMBER = {862832},
MRREVIEWER = {Thierry Fack},
       DOI = {10.1007/3-540-16777-3_74},
       URL = {http://dx.doi.org/10.1007/3-540-16777-3_74},
}

@article {BIST89,
    AUTHOR = {Bellissard, J. and Iochum, B. and Scoppola, E. and Testard, D.},
     TITLE = {Spectral properties of one-dimensional quasi-crystals},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {125},
      YEAR = {1989},
    NUMBER = {3},
     PAGES = {527--543},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {82A60 (47B39 81C05)},
  MRNUMBER = {1022526 (90m:82043)},
MRREVIEWER = {Hanna Nencka},
       URL = {http://projecteuclid.org/euclid.cmp/1104179532},
}

@article {BeVi90,
    AUTHOR = {Bellissard, J. and Vittot, M.},
     TITLE = {Heisenberg's picture and noncommutative geometry of the
              semiclassical limit in quantum mechanics},
   JOURNAL = {Ann. Inst. H. Poincar\'e Phys. Th\'eor.},
  FJOURNAL = {Annales de l'Institut Henri Poincar\'e. Physique Th\'eorique},
    VOLUME = {52},
      YEAR = {1990},
    NUMBER = {3},
     PAGES = {175--235},
      ISSN = {0246-0211},
     CODEN = {AHPAAO},
   MRCLASS = {81Q20 (46L60 46L87 58B30)},
  MRNUMBER = {1057445},
MRREVIEWER = {Mauro Spera},
       URL = {http://www.numdam.org/item?id=AIHPA_1990__52_3_175_0},
}

@incollection {Bel90,
    AUTHOR = {Bellissard, J.},
     TITLE = {Spectral properties of {S}chr\"odinger's operator with a
              {T}hue-{M}orse potential},
 BOOKTITLE = {Number theory and physics ({L}es {H}ouches, 1989)},
    SERIES = {Springer Proc. Phys.},
    VOLUME = {47},
     PAGES = {140--150},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1990},
   MRCLASS = {82B05 (19M05 47B39 47N55 54H20)},
  MRNUMBER = {1058456 (92b:82007)},
       DOI = {10.1007/978-3-642-75405-0_13},
       URL = {http://dx.doi.org/10.1007/978-3-642-75405-0_13},
}

@article {BIT91,
    AUTHOR = {Bellissard, J. and Iochum, B. and Testard, D.},
     TITLE = {Continuity properties of the electronic spectrum of {$1$}{D} quasicrystals},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {141},
      YEAR = {1991},
    NUMBER = {2},
     PAGES = {353--380},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {81Q10 (11Z50 47N50 81V70)},
  MRNUMBER = {1133271 (92j:81037)},
MRREVIEWER = {Guido A. Raggio},
       URL = {http://projecteuclid.org/euclid.cmp/1104248304},
}

@article {BeBoGh91,
    AUTHOR = {Bellissard, J. and Bovier, A. and Ghez, J. M.},
     TITLE = {Spectral properties of a tight binding {H}amiltonian with
              period doubling potential},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {135},
      YEAR = {1991},
    NUMBER = {2},
     PAGES = {379--399},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {81Q10 (47N50 47N55 58F40 82B28)},
  MRNUMBER = {1087389 (91m:81042)},
MRREVIEWER = {Helmut R{\"u}ssmann},
       URL = {http://projecteuclid.org/euclid.cmp/1104202031},
}

@incollection {Bel92,
    AUTHOR = {Bellissard, J.},
     TITLE = {Gap {L}abelling {T}heorems for {S}chr\"odinger operators},
 BOOKTITLE = {From number theo\-ry to physics ({L}es {H}ouches, 1989)},
     PAGES = {538--630},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1992},
   MRCLASS = {46L60 (19K14 19K56 19L64 46L55 46L80 81Q10 81V10)},
  MRNUMBER = {1221111 (94e:46120)},
MRREVIEWER = {Palle E. T. Jorgensen},
}

@incollection {Bel93,
    AUTHOR = {Bellissard, J.},
     TITLE = {The {G}ap {L}abelling {T}heorem: the case of automatic sequences},
 BOOKTITLE = {Quantum and non-commutative analysis ({K}yoto, 1992)},
    SERIES = {Math. Phys. Stud.},
    VOLUME = {16},
     PAGES = {179--181},
 PUBLISHER = {Kluwer Acad. Publ., Dordrecht},
      YEAR = {1993},
   MRCLASS = {46L60 (19K56 46N50 47B99 82B10)},
  MRNUMBER = {1276289},
}

@article {Bel94,
    AUTHOR = {Bellissard, J.},
     TITLE = {Lipshitz continuity of gap boundaries for {H}ofstadter-like
              spectra},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {160},
      YEAR = {1994},
    NUMBER = {3},
     PAGES = {599--613},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {46N50 (46L60 47N50 81Q10 81V10)},
  MRNUMBER = {1266066 (95c:46126)},
       URL = {http://projecteuclid.org/euclid.cmp/1104269713},
}

@article {BeScEl94,
    AUTHOR = {Bellissard, J. and van Elst, A. and Schulz-Baldes, H.},
     TITLE = {The noncommutative geometry of the quantum {H}all effect},
      NOTE = {Topology and physics},
   JOURNAL = {J. Math. Phys.},
  FJOURNAL = {Journal of Mathematical Physics},
    VOLUME = {35},
      YEAR = {1994},
    NUMBER = {10},
     PAGES = {5373--5451},
      ISSN = {0022-2488},
     CODEN = {JMAPAQ},
   MRCLASS = {81V70 (46L60 46L87 58B30 82D45)},
  MRNUMBER = {1295473},
MRREVIEWER = {Albert Jeu-Liang Sheu},
       DOI = {10.1063/1.530758},
       URL = {http://dx.doi.org/10.1063/1.530758},
}

@incollection {BeHeZa00,
    AUTHOR = {Bellissard, J. and Herrmann, D. J. L. and Zarrouati, M.},
     TITLE = {Hulls of aperiodic solids and gap labeling theorems},
 BOOKTITLE = {Directions in mathematical quasicrystals},
    SERIES = {CRM Monogr. Ser.},
    VOLUME = {13},
     PAGES = {207--258},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2000},
   MRCLASS = {82D20 (19K14 52C23 81R60 82D25)},
  MRNUMBER = {1798994},
MRREVIEWER = {Johannes Kellendonk},
}

@Inbook {Bel02,
   author = {Bellissard, J.},
    title = {Coherent and Dissipative Transport in Aperiodic Solids: An Overview},
booktitle = {Dynamics of Dissipation},
     year = {2002},
publisher = {Springer Berlin Heidelberg},
  address = {Berlin, Heidelberg},
    pages = {413--485},
     isbn = {978-3-540-46122-7},
      doi = {10.1007/3-540-46122-1_18},
      url = {http://dx.doi.org/10.1007/3-540-46122-1_18},
}

@incollection {Bel03,
    AUTHOR = {Bellissard, J.},
     TITLE = {The noncommutative geometry of aperiodic solids},
 BOOKTITLE = {Geometric and topological methods for quantum field theory
              ({V}illa de {L}eyva, 2001)},
     PAGES = {86--156},
 PUBLISHER = {World Sci. Publ., River Edge, NJ},
      YEAR = {2003},
   MRCLASS = {81Q70 (58B34 82C10)},
  MRNUMBER = {2009996},
       DOI = {10.1142/9789812705068_0002},
       URL = {http://dx.doi.org/10.1142/9789812705068_0002},
}

@article {BeBeGa06,
    AUTHOR = {Bellissard, J. and Benedetti, R. and Gambaudo,
              J.-M.},
     TITLE = {Spaces of tilings, finite telescopic approximations and
              gap-labeling},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {261},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {1--41},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {46L55 (19K14 37B50 47B80 52C23 82B44)},
  MRNUMBER = {2193205 (2007c:46063)},
MRREVIEWER = {John Hunton},
       DOI = {10.1007/s00220-005-1445-z},
       URL = {http://dx.doi.org/10.1007/s00220-005-1445-z},
}

@article {BeRaSh10,
    AUTHOR = {Bellissard, J. and Radin, C. and Shlosman, S.},
     TITLE = {The characterization of ground states},
   JOURNAL = {J. Phys. A},
  FJOURNAL = {Journal of Physics. A. Mathematical and Theoretical},
    VOLUME = {43},
      YEAR = {2010},
    NUMBER = {30},
     PAGES = {305001, 7},
      ISSN = {1751-8113},
   MRCLASS = {82B21 (60K35 82B05)},
  MRNUMBER = {2659612},
MRREVIEWER = {Massimo Campanino},
       DOI = {10.1088/1751-8113/43/30/305001},
       URL = {http://dx.doi.org/10.1088/1751-8113/43/30/305001},
}


@article {BeQuSh13,
    AUTHOR = {Ben-Abraham, S. I. and Quandt, A. and Shapira, D.},
     TITLE = {Multidimensional paperfolding systems},
   JOURNAL = {Acta Crystallogr. Sect. A},
  FJOURNAL = {Acta Crystallographica Section A. Foundations of
              Crystallography},
    VOLUME = {69},
      YEAR = {2013},
    NUMBER = {2},
     PAGES = {123--130},
      ISSN = {0108-7673},
   MRCLASS = {52C23},
  MRNUMBER = {3027748},
       DOI = {10.1107/S010876731204531X},
       URL = {http://dx.doi.org/10.1107/S010876731204531X},
}

@article {BeOy02,
    AUTHOR = {Benameur, M.-T. and Oyono-Oyono, H.},
     TITLE = {Calcul du label des gaps pour les quasi-cristaux},
   JOURNAL = {C. R. Math. Acad. Sci. Paris},
  FJOURNAL = {Comptes Rendus Math\'ematique. Acad\'emie des Sciences. Paris},
    VOLUME = {334},
      YEAR = {2002},
    NUMBER = {8},
     PAGES = {667--670},
      ISSN = {1631-073X},
   MRCLASS = {52C23 (37B10 37B50)},
  MRNUMBER = {1903367},
MRREVIEWER = {David Damanik},
       DOI = {10.1016/S1631-073X(02)02312-9},
       URL = {http://dx.doi.org/10.1016/S1631-073X(02)02312-9},
}

@article {BeOy07,
    AUTHOR = {Benameur, M.-T. and Oyono-Oyono, H.},
     TITLE = {Index theory for quasi-crystals. {I}. {C}omputation of the
              gap-label group},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {252},
      YEAR = {2007},
    NUMBER = {1},
     PAGES = {137--170},
      ISSN = {0022-1236},
     CODEN = {JFUAAW},
   MRCLASS = {58J22 (19K56 52C23 58B34)},
  MRNUMBER = {2357353},
MRREVIEWER = {Nicolae Cotfas},
       DOI = {10.1016/j.jfa.2006.03.029},
       URL = {http://dx.doi.org/10.1016/j.jfa.2006.03.029},
}

@article {BeGa03,
    AUTHOR = {Benedetti, R. and Gambaudo, J.-M.},
     TITLE = {On the dynamics of {$\mathbb{G}$}-solenoids. {A}pplications to
              {D}elone sets},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {23},
      YEAR = {2003},
    NUMBER = {3},
     PAGES = {673--691},
      ISSN = {0143-3857},
   MRCLASS = {37B99 (37A15 37B50 37C40 37C85 52C23)},
  MRNUMBER = {1992658},
       DOI = {10.1017/S0143385702001578},
       URL = {http://dx.doi.org/10.1017/S0143385702001578},
}

@article {BeSi91,
    title = {Band spectrum of the octagonal quasicrystal: Finite measure, gaps, and chaos},
   author = {Benza, V. G. and Sire, C.},
  journal = {Phys. Rev. B},
   volume = {44},
    issue = {18},
    pages = {10343--10345},
 numpages = {0},
     year = {1991},
    month = {Nov},
publisher = {American Physical Society},
      doi = {10.1103/PhysRevB.44.10343},
      url = {http://link.aps.org/doi/10.1103/PhysRevB.44.10343},
}


@article {Ber66,
    AUTHOR = {Berger, R.},
     TITLE = {The undecidability of the domino problem},
   JOURNAL = {Mem. Amer. Math. Soc. No.},
  FJOURNAL = {Memoirs of the American Mathematical Society},
    VOLUME = {66},
      YEAR = {1966},
     PAGES = {72},
      ISSN = {0065-9266},
   MRCLASS = {02.74},
  MRNUMBER = {0216954},
MRREVIEWER = {J. R. B{\"u}chi},
}

@article{BeMaCyKlLa93,
    title = {Evidence for unconventional electronic transport in quasicrystals},
   author = {Mayou, D. and Berger, C. and Cyrot-Lackmann, F. and Klein, T. and Lanco, P.},
  journal = {Phys. Rev. Lett.},
   volume = {70},
    issue = {25},
    pages = {3915--3918},
 numpages = {0},
     year = {1993},
    month = {Jun},
publisher = {American Physical Society},
      doi = {10.1103/PhysRevLett.70.3915},
      url = {http://link.aps.org/doi/10.1103/PhysRevLett.70.3915},
}

@Inbook {Ber94,
    AUTHOR = {Berger, C.},
     TITLE = {Electronic properties of quasicrystals},
 BOOKTITLE = {Lectures on Quasicrystals},
     NOTES = {by Hippert, F., Gratias, D.},
 PUBLISHER = {Les Editions de Physique},
    ADRESS = {Les Ulis},
     PAGES = {463--504},
      ISBN = {9782868832306},
      YEAR = {1994},
}

@article {BeMa12,
    AUTHOR = {Belmonte, F. and M{\u{a}}ntoiu, M.},
     TITLE = {Covariant fields of {${C}^{\ast}$}-algebras under {R}ieffel
              deformation},
   JOURNAL = {SIGMA Symmetry Integrability Geom. Methods Appl.},
  FJOURNAL = {SIGMA. Symmetry, Integrability and Geometry. Methods and
              Applications},
    VOLUME = {8},
      YEAR = {2012},
     PAGES = {Paper 091, 12},
      ISSN = {1815-0659},
   MRCLASS = {46L65 (35S05 47C15 81Q10)},
  MRNUMBER = {3007268},
MRREVIEWER = {Yuri A. Kordyukov},
       DOI = {10.3842/SIGMA.2012.091},
       URL = {http://dx.doi.org/10.3842/SIGMA.2012.091},
}

@misc {BjHaPo16,
    AUTHOR = {Bj{\"o}rklund, M. and Hartnick, T. and Pogorzelski, F.},
     TITLE = {{A}periodic order and spherical diffraction},
      NOTE = {arXiv:1602.0892},
      YEAR = {2016},
       URL = {http://arxiv.org/pdf/1602.08928v1.pdf},
}

@article {Bla96,
    AUTHOR = {Blanchard, {\'E}.},
     TITLE = {D\'eformations de {${C}^{\ast}$}-alg\`ebres de {H}opf},
   JOURNAL = {Bull. Soc. Math. France},
  FJOURNAL = {Bulletin de la Soci\'et\'e Math\'ematique de France},
    VOLUME = {124},
      YEAR = {1996},
    NUMBER = {1},
     PAGES = {141--215},
      ISSN = {0037-9484},
     CODEN = {BSMFAA},
   MRCLASS = {46L05 (16W30 46L30 46L45 46L60 46L87 58B30 81R50)},
  MRNUMBER = {1395009 (97f:46092)},
MRREVIEWER = {Albert Jeu-Liang Sheu},
       URL = {http://www.numdam.org/item?id=BSMF_1996__124_1_141_0},
}

@article {BoGhEr93,
    AUTHOR = {Bovier, A. and Ghez, J. M.},
     TITLE = {Erratum: ``{S}pectral properties of one-dimensional
              {S}chr\"odinger operators with potentials generated by
              substitutions'' [{C}omm.\ {M}ath.\ {P}hys.\ {\bf 158} (1993),
              no.\ 1, 45--66; {MR}1243715 (94k:82064)]},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {166},
      YEAR = {1994},
    NUMBER = {2},
     PAGES = {431--432},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {82C10 (47B39 47N55)},
  MRNUMBER = {1309558 (95j:82033)},
       URL = {http://projecteuclid.org/euclid.cmp/1104271618},
}

@article {BoGh93,
    AUTHOR = {Bovier, A. and Ghez, J. M.},
     TITLE = {Spectral properties of one-dimensional {S}chr\"odinger
              operators with potentials generated by substitutions},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {158},
      YEAR = {1993},
    NUMBER = {1},
     PAGES = {45--66},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {82C10 (47B39 47N55)},
  MRNUMBER = {1243715 (94k:82064)},
MRREVIEWER = {G. V. Rozenblyum},
       URL = {http://projecteuclid.org/euclid.cmp/1104254130},
}

@article {BoEmSo03,
    AUTHOR = {B{\"o}ttcher, A. and Embree, M. and Sokolov, V. I.},
     TITLE = {The spectra of large {T}oeplitz band matrices with a randomly
              perturbed entry},
   JOURNAL = {Math. Comp.},
  FJOURNAL = {Mathematics of Computation},
    VOLUME = {72},
      YEAR = {2003},
    NUMBER = {243},
     PAGES = {1329--1348 (electronic)},
      ISSN = {0025-5718},
     CODEN = {MCMPAF},
   MRCLASS = {15A42 (15A18 47A10 47B35 47B80)},
  MRNUMBER = {1972739 (2004c:15032)},
       DOI = {10.1090/S0025-5718-03-01505-9},
       URL = {http://dx.doi.org/10.1090/S0025-5718-03-01505-9},
}

@incollection {BoGrSp03,
    AUTHOR = {B{\"o}ttcher, A. and Grudsky, S. and Spitkovsky,
              I.},
     TITLE = {On the essential spectrum of {T}oeplitz operators with
              semi-almost periodic symbols},
 BOOKTITLE = {Singular integral operators, factorization and applications},
    SERIES = {Oper. Theory Adv. Appl.},
    VOLUME = {142},
     PAGES = {59--77},
 PUBLISHER = {Birkh\"auser, Basel},
      YEAR = {2003},
   MRCLASS = {47B35 (47A10)},
  MRNUMBER = {2167360 (2006i:47048)},
MRREVIEWER = {R. V. Duduchava},
}

@misc {BrLi11,
    AUTHOR = {le Bris, C. and Lions, P. L.},
     TITLE = {Some recent progress in deterministic and stochastic homogenization of elliptic {PDE}'s},
      YEAR = {September 5-6,2011},
      Note = {talk given at the conference Modern Trends in PDE’s, Geometric Analysis and Mathematical Physics, Cergy-Pontoise, France.},
}

@article {Bru46,
    AUTHOR = {de Bruijn, N. G.},
     TITLE = {A combinatorial problem},
   JOURNAL = {Nederl. Akad. Wetensch., Proc.},
    VOLUME = {49},
      YEAR = {1946},
     PAGES = {758--764 = Indagationes Math. 8, 461--467 (1946)},
   MRCLASS = {09.0X},
  MRNUMBER = {0018142 (8,247d)},
MRREVIEWER = {J. Riordan},
}

@article {Bun06,
    AUTHOR = {Buneci, M. R.},
     TITLE = {Groupoid {${C}^{\ast}$}-algebras},
   JOURNAL = {Surv. Math. Appl.},
  FJOURNAL = {Surveys in Mathematics and its Applications},
    VOLUME = {1},
      YEAR = {2006},
     PAGES = {71--98 (electronic)},
      ISSN = {1842-6298},
   MRCLASS = {46L05 (22D25 46L55)},
  MRNUMBER = {2274294 (2007h:46067)},
}

@article {CaKlMa87,
    AUTHOR = {Carmona, R. and Klein, A. and Martinello, F.},
     TITLE = {Anderson localization for {B}ernoulli and other singular
              potentials},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {108},
      YEAR = {1987},
    NUMBER = {1},
     PAGES = {41--66},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {82A57 (60K35 82A05)},
  MRNUMBER = {872140},
MRREVIEWER = {Massimo Campanino},
       URL = {http://projecteuclid.org/euclid.cmp/1104116357},
}

@misc {CaPe15,
    AUTHOR = {Carroll, D. and Penland A.},
     TITLE = {Periodic points on shifts of finite type and commensurability invariants of groups},
      NOTE = {arXiv:1502.03195},
      YEAR = {2015},
       URL = {http://arxiv.org/abs/1502.03195},
}

@article {Cas97,
    AUTHOR = {Cassaigne, J.},
     TITLE = {Complexit\'e et facteurs sp\'eciaux},
      NOTE = {Journ{\'e}es Montoises (Mons, 1994)},
   JOURNAL = {Bull. Belg. Math. Soc. Simon Stevin},
  FJOURNAL = {Bulletin of the Belgian Mathematical Society. Simon Stevin},
    VOLUME = {4},
      YEAR = {1997},
    NUMBER = {1},
     PAGES = {67--88},
      ISSN = {1370-1444},
   MRCLASS = {68R15 (11B85)},
  MRNUMBER = {1440670 (98c:68176)},
MRREVIEWER = {Jean-Paul Allouche},
       URL = {http://projecteuclid.org/euclid.bbms/1105730624},
}

@article {Cha50,
    AUTHOR = {Chabauty, C.},
     TITLE = {Limite d'ensembles et g\'eom\'etrie des nombres},
   JOURNAL = {Bull. Soc. Math. France},
  FJOURNAL = {Bulletin de la Soci\'et\'e Math\'ematique de France},
    VOLUME = {78},
      YEAR = {1950},
     PAGES = {143--151},
      ISSN = {0037-9484},
   MRCLASS = {20.0X},
  MRNUMBER = {0038983 (12,479f)},
MRREVIEWER = {I. E. Segal},
}

@article {Cha69,
    AUTHOR = {Chacon, R. V.},
     TITLE = {Weakly mixing transformations which are not strongly mixing},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {22},
      YEAR = {1969},
     PAGES = {559--562},
      ISSN = {0002-9939},
   MRCLASS = {28.70},
  MRNUMBER = {0247028},
MRREVIEWER = {J. E. Marsden},
}

@article {ChSiLi13,
    AUTHOR = {Chandler-Wilde, S. N. and Chonchaiya, R. and
              Lindner, M.},
     TITLE = {On the spectra and pseudospectra of a class of
              non-self-adjoint random matrices and operators},
   JOURNAL = {Oper. Matrices},
  FJOURNAL = {Operators and Matrices},
    VOLUME = {7},
      YEAR = {2013},
    NUMBER = {4},
     PAGES = {739--775},
      ISSN = {1846-3886},
   MRCLASS = {47A10 (47B80)},
  MRNUMBER = {3154570},
MRREVIEWER = {Lyonell S. Boulton},
       DOI = {10.7153/oam-07-43},
       URL = {http://dx.doi.org/10.7153/oam-07-43},
}

@article {ChLi08,
    AUTHOR = {Chandler-Wilde, Simon N. and Lindner, M.},
     TITLE = {Sufficiency of {F}avard's condition for a class of
              band-dominated operators on the axis},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {254},
      YEAR = {2008},
    NUMBER = {4},
     PAGES = {1146--1159},
      ISSN = {0022-1236},
     CODEN = {JFUAAW},
   MRCLASS = {47A05 (47A10 47A53 47B37)},
  MRNUMBER = {2381205 (2008k:47003)},
MRREVIEWER = {Steffen Roch},
       DOI = {10.1016/j.jfa.2007.09.004},
       URL = {http://dx.doi.org/10.1016/j.jfa.2007.09.004},
}

@article {Cec37,
    AUTHOR = {{\v{C}}ech, E.},
     TITLE = {On bicompact spaces},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {38},
      YEAR = {1937},
    NUMBER = {4},
     PAGES = {823--844},
      ISSN = {0003-486X},
     CODEN = {ANMAAH},
   MRCLASS = {Contributed Item},
  MRNUMBER = {1503374},
       DOI = {10.2307/1968839},
       URL = {http://dx.doi.org/10.2307/1968839},
}


@article {Chi08,
    AUTHOR = {Chierchia, L.},
     TITLE = {A. {N}. {K}olmogorov's 1954 paper on nearly-integrable {H}amiltonian systems. {A} comment on: ``{O}n conservation of
              conditionally periodic motions for a small change in {H}amilton's function'' [{D}okl. {A}kad. {N}auk {SSSR} ({N}.{S}.) 
              {\bf 98} (1954), 527--530; MR0068687]},
   JOURNAL = {Regul. Chaotic Dyn.},
  FJOURNAL = {Regular and Chaotic Dynamics. International Scientific Journal},
    VOLUME = {13},
      YEAR = {2008},
    NUMBER = {2},
     PAGES = {130--139},
      ISSN = {1560-3547},
   MRCLASS = {37J40 (70H08)},
  MRNUMBER = {2395530},
       DOI = {10.1134/S1560354708020056},
       URL = {http://dx.doi.org/10.1134/S1560354708020056},
}

@article {CuKa95,
    AUTHOR = {Culik, II, K. and Kari, J.},
     TITLE = {An aperiodic set of {W}ang cubes},
   JOURNAL = {J.UCS},
  FJOURNAL = {J.UCS. The Journal of Universal Computer Science},
    VOLUME = {1},
      YEAR = {1995},
    NUMBER = {10},
     PAGES = {675--686 (electronic)},
      ISSN = {0948-6968},
   MRCLASS = {68R05 (05B45 68Q65 68Q80)},
  MRNUMBER = {1392428},
}

@misc {Coh14,
    AUTHOR = {Cohen, D. B.},
     TITLE = {The large scale geometry of strongly aperiodic subshifts of finite},
      NOTE = {arXiv:1412.4572},
      YEAR = {2014},
       URL = {http://arxiv.org/abs/1412.4572},
}

@incollection {Con78,
    AUTHOR = {Connes, A.},
     TITLE = {Sur la th\'{e}orie non commutative de l'int\'{e}gration},
 BOOKTITLE = {Alg\`{e}bres d'op\'{e}rateurs ({S}\'{e}m., {L}es {P}lans-sur-{B}ex,
              1978)},
    SERIES = {Lecture Notes in Math.},
    VOLUME = {725},
     PAGES = {19--143},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1979},
   MRCLASS = {46L50 (22E46 58G10 58G12)},
  MRNUMBER = {548112 (81g:46090)},
MRREVIEWER = {M. F. Atiyah},
}

@article {CoPu15,
    AUTHOR = {Cornean, H. D. and Purice, R.},
     TITLE = {Spectral edge regularity of magnetic {H}amiltonians},
   JOURNAL = {J. Lond. Math. Soc. (2)},
  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {92},
      YEAR = {2015},
    NUMBER = {1},
     PAGES = {89--104},
      ISSN = {0024-6107},
   MRCLASS = {47A55 (35J10 35Q40 81V10)},
  MRNUMBER = {3384506},
       DOI = {10.1112/jlms/jdv019},
       URL = {http://dx.doi.org/10.1112/jlms/jdv019},
}

@article {CoHe73,
    AUTHOR = {Coven, E. M. and Hedlund, G. A.},
     TITLE = {Sequences with minimal block growth},
   JOURNAL = {Math. Systems Theory},
  FJOURNAL = {Mathematical Systems Theory. An International Journal on
              Mathematical Computing Theory},
    VOLUME = {7},
      YEAR = {1973},
     PAGES = {138--153},
      ISSN = {0025-5661},
   MRCLASS = {54H20},
  MRNUMBER = {0322838},
MRREVIEWER = {R. Ellis},
}

@article {DaNeSh99,
    AUTHOR = {Dahmen, K. A. and Nelson, D. R. and Shnerb, N. M.},
     TITLE = {Population dynamics and non-Hermitian localization},
  FJOURNAL = {Statistical Mechanics of Biocomplexity, Lecture Notes in Physics},
    VOLUME = {527},
      YEAR = {1999},
     PAGES = {124--151},
       DOI = {10.1007/BFb0105012},
}

@incollection {Dam00Gord,
    AUTHOR = {Damanik, D.},
     TITLE = {Gordon-type arguments in the spectral theory of
              one-dimensional quasicrystals},
 BOOKTITLE = {Directions in mathematical quasicrystals},
    SERIES = {CRM Monogr. Ser.},
    VOLUME = {13},
     PAGES = {277--305},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2000},
   MRCLASS = {81Q10 (47B39 47N55 52C23)},
  MRNUMBER = {1798997 (2002c:81048)},
MRREVIEWER = {Jean-Michel Ghez},
}

@article {Dam98PerDoub,
    AUTHOR = {Damanik, D.},
     TITLE = {Singular continuous spectrum for the period doubling
              {H}amiltonian on a set of full measure},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {196},
      YEAR = {1998},
    NUMBER = {2},
     PAGES = {477--483},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {81Q10 (47B39 47N50 82B44)},
  MRNUMBER = {1645023 (99i:81035)},
MRREVIEWER = {Oliver Knill},
       DOI = {10.1007/s002200050432},
       URL = {http://dx.doi.org/10.1007/s002200050432},
}

@article {Dam98,
    AUTHOR = {Damanik, D.},
     TITLE = {Singular continuous spectrum for a class of substitution
              {H}amiltonians},
   JOURNAL = {Lett. Math. Phys.},
  FJOURNAL = {Letters in Mathematical Physics. A Journal for the Rapid
              Dissemination of Short Contributions in the Field of
              Mathematical Physics},
    VOLUME = {46},
      YEAR = {1998},
    NUMBER = {4},
     PAGES = {303--311},
      ISSN = {0377-9017},
     CODEN = {LMPHDY},
   MRCLASS = {81Q10 (47B39 47N50)},
  MRNUMBER = {1668569 (99m:81053)},
MRREVIEWER = {Jean-Michel Ghez},
       DOI = {10.1023/A:1007510721504},
       URL = {http://dx.doi.org/10.1023/A:1007510721504},
}

@article {Dam00Sing,
    AUTHOR = {Damanik, D.},
     TITLE = {Singular continuous spectrum for a class of substitution
              {H}amiltonians. {II}},
   JOURNAL = {Lett. Math. Phys.},
  FJOURNAL = {Letters in Mathematical Physics. A Journal for the Rapid
              Dissemination of Short Contributions in the Field of
              Mathematical Physics},
    VOLUME = {54},
      YEAR = {2000},
    NUMBER = {1},
     PAGES = {25--31},
      ISSN = {0377-9017},
     CODEN = {LMPHDY},
   MRCLASS = {81Q10 (47B39 47N50)},
  MRNUMBER = {1846720 (2002g:81027)},
MRREVIEWER = {Jean-Michel Ghez},
       DOI = {10.1023/A:1007697301341},
       URL = {http://dx.doi.org/10.1023/A:1007697301341},
}

@incollection {Dam07,
    AUTHOR = {Damanik, D.},
     TITLE = {Strictly ergodic subshifts and associated operators},
 BOOKTITLE = {Spectral theory and mathematical physics: a {F}estschrift in
              honor of {B}arry {S}imon's 60th birthday},
    SERIES = {Proc. Sympos. Pure Math.},
    VOLUME = {76},
     PAGES = {505--538},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2007},
   MRCLASS = {47B36 (37A99 37B10 47B80 47N50 81Q10 82B44)},
  MRNUMBER = {2307746},
MRREVIEWER = {T{\'u}lio O. Carvalho},
       DOI = {10.1090/pspum/076.2/2307746},
       URL = {http://dx.doi.org/10.1090/pspum/076.2/2307746},
}

@misc {DaGo08,
    AUTHOR = {Damanik, D. and Gorodetski, A.},
     TITLE = {The Spectrum and the spectral type of the off-diagonal Fibonacci operator},
      NOTE = {arXiv:0807.3024},
      YEAR = {2008},
       URL = {http://arxiv.org/abs/0807.3024},
}

@misc {Dam09,
    AUTHOR = {Damanik, D.},
     TITLE = {The Spectrum of the Almost Mathieu Operator},
      NOTE = {arXiv:0908.1093},
      YEAR = {2009},
       URL = {http://arxiv.org/abs/0908.1093},
}

@article {DaGo11,
    AUTHOR = {Damanik, D. and Gorodetski, A.},
     TITLE = {Spectral and quantum dynamical properties of the weakly
              coupled {F}ibonacci {H}amiltonian},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {305},
      YEAR = {2011},
    NUMBER = {1},
     PAGES = {221--277},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {81Q10 (47B36 47B80 47N50)},
  MRNUMBER = {2802305 (2012g:81065)},
       DOI = {10.1007/s00220-011-1220-2},
       URL = {http://dx.doi.org/10.1007/s00220-011-1220-2},
}

@article {DaLe99I,
    AUTHOR = {Damanik, D. and Lenz, D.},
     TITLE = {Uniform spectral properties of one-dimensional quasicrystals.
              {I}. {A}bsence of eigenvalues},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {207},
      YEAR = {1999},
    NUMBER = {3},
     PAGES = {687--696},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {81Q10 (47B39 47N55)},
  MRNUMBER = {1727235 (2000k:81078)},
MRREVIEWER = {Jean-Michel Ghez},
       DOI = {10.1007/s002200050742},
       URL = {http://dx.doi.org/10.1007/s002200050742},
}

@article {DaLe99II,
    AUTHOR = {Damanik, D. and Lenz, D.},
     TITLE = {Uniform spectral properties of one-dimensional quasicrystals.
              {II}. {T}he {L}yapunov exponent},
   JOURNAL = {Lett. Math. Phys.},
  FJOURNAL = {Letters in Mathematical Physics. A Journal for the Rapid
              Dissemination of Short Contributions in the Field of
              Mathematical Physics},
    VOLUME = {50},
      YEAR = {1999},
    NUMBER = {4},
     PAGES = {245--257},
      ISSN = {0377-9017},
     CODEN = {LMPHDY},
   MRCLASS = {81Q10 (47B39 47B80 47N55)},
  MRNUMBER = {1768702 (2001g:81060)},
MRREVIEWER = {Jean-Michel Ghez},
       DOI = {10.1023/A:1007614218486},
       URL = {http://dx.doi.org/10.1023/A:1007614218486},
}

@article {Dam00,
    AUTHOR = {Damanik, D.},
     TITLE = {Local symmetries in the period-doubling sequence},
   JOURNAL = {Discrete Appl. Math.},
  FJOURNAL = {Discrete Applied Mathematics. The Journal of Combinatorial
              Algorithms, Informatics and Computational Sciences},
    VOLUME = {100},
      YEAR = {2000},
    NUMBER = {1-2},
     PAGES = {115--121},
      ISSN = {0166-218X},
     CODEN = {DAMADU},
   MRCLASS = {68R15 (11B83)},
  MRNUMBER = {1733386},
       DOI = {10.1016/S0166-218X(99)00199-7},
       URL = {http://dx.doi.org/10.1016/S0166-218X(99)00199-7},
}

@article {DaLeKi00,
    AUTHOR = {Damanik, D. and Killip, R. and Lenz, D.},
     TITLE = {Uniform spectral properties of one-dimensional quasicrystals.
              {III}. {$\alpha$}-continuity},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {212},
      YEAR = {2000},
    NUMBER = {1},
     PAGES = {191--204},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {81Q10 (39A70 47B36 47B39 47N55)},
  MRNUMBER = {1764367 (2001g:81061)},
MRREVIEWER = {Jean-Michel Ghez},
       DOI = {10.1007/s002200000203},
       URL = {http://dx.doi.org/10.1007/s002200000203},
}

@misc {DaLiQu14,
    AUTHOR = {Damanik, D. and Liu, Q.-H. and Qu, Y.-H.},
     TITLE = {Schr\"odinger {O}perators with {D}ynami\-cally {D}efined {P}otentials: {A} {S}urvey},
      NOTE = {	arXiv:1410.2445},
      YEAR = {2014},
       URL = {http://arxiv.org/abs/1410.2445},
}

@inbook {DaEmGo15,
    AUTHOR = {Damanik, D. and Embree, M. and Gorodetski, A.},
     TITLE = {Spectral properties of {S}chr{\"o}\-dinger operators arising in
              the study of quasicrystals},
 BOOKTITLE = {Mathematics of aperiodic order},
    SERIES = {Prog. Math. Phys.},
    VOLUME = {309},
     PAGES = {307--370},
 PUBLISHER = {Birkh{\"a}user Springer, Basel},
      YEAR = {2015},
   MRCLASS = {81Q10 (35J10 35P05 37J99 47B36)},
  MRNUMBER = {3381485},
}

@article {DaGoSo13,
    AUTHOR = {Damanik, D. and Gorodetski, A. and Solomyak, B.},
     TITLE = {Absolutely continuous convolutions of singular measures and an
              application to the square {F}ibonacci {H}amiltonian},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {164},
      YEAR = {2015},
    NUMBER = {8},
     PAGES = {1603--1640},
      ISSN = {0012-7094},
   MRCLASS = {47N50 (37C45 47B36 81Q10)},
  MRNUMBER = {3352042},
       DOI = {10.1215/00127094-3119739},
       URL = {http://dx.doi.org/10.1215/00127094-3119739},
}


@misc {DaGo16,
    AUTHOR = {Damanik, D. and Gorodetski, A.},
     TITLE = {Sums of regular Cantor sets of large dimension and the Square Fibonacci Hamiltonian},
      YEAR = {2016},
      NOTE = {arXiv:1601.01639},
       URL = {http://arxiv.org/abs/1601.01639},
}

@misc {DaLiQu15,
    AUTHOR = {Damanik, D. and Liu, Q.-H. and Qu, Y.-H.},
     TITLE = {Spectral properties of {S}chr{\"o}dinger operators with pattern sturmian potentials},
      NOTE = {arXiv:1511.03834},
      YEAR = {2015},
       URL = {http://de.arxiv.org/abs/1511.03834v1},
}

@article {DaGoLiQu15,
    AUTHOR = {Damanik, D. and Gorodetski, A. and Liu, Q.-H. and Qu,
              Y.-H.},
     TITLE = {Transport exponents of {S}turmian {H}amiltonians},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {269},
      YEAR = {2015},
    NUMBER = {5},
     PAGES = {1404--1440},
      ISSN = {0022-1236},
   MRCLASS = {35J10 (35B15)},
  MRNUMBER = {3369942},
MRREVIEWER = {Alessandro Selvitella},
       DOI = {10.1016/j.jfa.2015.05.018},
       URL = {http://dx.doi.org/10.1016/j.jfa.2015.05.018},
}

@article {Dav01,
    AUTHOR = {Davies, E. B.},
     TITLE = {Spectral theory of pseudo-ergodic operators},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {216},
      YEAR = {2001},
    NUMBER = {3},
     PAGES = {687--704},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {47B80 (47A10 47B39 47N55 47N60 81Q10 82B44)},
  MRNUMBER = {1815722 (2002g:47076)},
MRREVIEWER = {J. A. Van Casteren},
       DOI = {10.1007/s002200000352},
       URL = {http://dx.doi.org/10.1007/s002200000352},
}

@article {Dea95,
    AUTHOR = {Deaconu, V.},
     TITLE = {Groupoids associated with endomorphisms},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {347},
      YEAR = {1995},
    NUMBER = {5},
     PAGES = {1779--1786},
      ISSN = {0002-9947},
     CODEN = {TAMTAM},
   MRCLASS = {46L55 (19K99 20L15 46L80 54H20 57N10)},
  MRNUMBER = {1233967 (95h:46104)},
MRREVIEWER = {Alain Valette},
       DOI = {10.2307/2154972},
       URL = {http://dx.doi.org/10.2307/2154972},
}

@article {DWM13,
    AUTHOR = {Dean, C.R. and Wang, L. and Maher, P. and Forsythe, C. and Ghahari, F. and Gao, Y. and Katoch, J. and Ishigami, M. and Moon, P. and Koshino, M. and Taniguchi, T. and Watanabe, K. and Shepard, K.L. and Hone, J. and Kim, P.},
     TITLE = {Hofstadter's butterfly and the fractal quantum {H}all effect in moir\'{e} superlattices},
   JOURNAL = {Nature},
    VOLUME = {497},
      YEAR = {2013},
     PAGES = {598--602},
   MRCLASS = {497IS (7451SP 598EP 602PB)},
       DOI = {10.1038/nature12186},
       URL = {http://www.nature.com/nature/journal/v497/n7451/abs/nature12186.html#supplementary-information
ER},
}

@article {DiNa08,
    AUTHOR = {Di Maio, G. and Naimpally, S.},
     TITLE = {Hit-and-far-miss topologies},
   JOURNAL = {Mat. Vesnik},
  FJOURNAL = {Matematichki Vesnik},
    VOLUME = {60},
      YEAR = {2008},
    NUMBER = {1},
     PAGES = {59--78},
      ISSN = {0025-5165},
   MRCLASS = {54B20 (54E05 54E15)},
  MRNUMBER = {2403272},
MRREVIEWER = {Jiling Cao},
}

@article {DiDo63,
    AUTHOR = {Dixmier, J. and Douady, A.},
     TITLE = {Champs continus d'espaces hilbertiens et de {${C}^{\ast}$}-alg\`ebres},
   JOURNAL = {Bull. Soc. Math. France},
  FJOURNAL = {Bulletin de la Soci\'et\'e Math\'ematique de France},
    VOLUME = {91},
      YEAR = {1963},
     PAGES = {227--284},
      ISSN = {0037-9484},
   MRCLASS = {46.65 (22.60)},
  MRNUMBER = {0163182 (29 \#485)},
MRREVIEWER = {J. M. G. Fell},
}

@article {Dru00a,
    AUTHOR = {Drude, P.},
     TITLE = {Zur {E}lektronentheorie der {M}etalle},
   JOURNAL = {Ann. Phys.},
  FJOURNAL = {Annalen der Physik},
    VOLUME = {306},
     ISSUE = {3},
      YEAR = {1900},
     PAGES = {566--613},
       DOI = {10.1002/andp.19003060312},
}

@article {Dru00b,
    AUTHOR = {Drude, P.},
     TITLE = {{Z}ur {E}lektronentheorie der {M}etalle; {II}. {T}eil. {G}alvanomagnetische und thermomagnetische {E}ffecte},
   JOURNAL = {Ann. Phys.},
  FJOURNAL = {Annalen der Physik},
    VOLUME = {308},
     ISSUE = {11},
      YEAR = {1900},
     PAGES = {369--402},
       DOI = {10.1002/andp.19003081102},
}

@misc {DuKa85,
    AUTHOR = {Duneau, M. and Katz, A.},
     TITLE = {Quasiperiodic patterns},
   JOURNAL = {Phys. Rev. Lett.},
  FJOURNAL = {Physical Review Letters},
    VOLUME = {54},
      YEAR = {1985},
    NUMBER = {25},
     PAGES = {2688--2691},
      ISSN = {0031-9007},
     CODEN = {PRLTAO},
   MRCLASS = {52A45 (05B45 82A60)},
  MRNUMBER = {791727},
       DOI = {10.1103/PhysRevLett.54.2688},
       URL = {http://dx.doi.org/10.1103/PhysRevLett.54.2688},
}

@misc {DuKa86,
    AUTHOR = {Duneau, M. and Katz, A.},
     TITLE = {Quasiperiodic patterns and icosahedral symmetry},
   JOURNAL = {J. Physique},
  FJOURNAL = {Le Journal de Physique},
    VOLUME = {47},
      YEAR = {1986},
    NUMBER = {2},
     PAGES = {181--196},
      ISSN = {0302-0738},
     CODEN = {JOPQAG},
   MRCLASS = {52A45 (05B45 82A60)},
  MRNUMBER = {831883},
MRREVIEWER = {Egon Schulte},
}

@article {EhLeRo75,
    AUTHOR = {Ehrenfeucht, A. and Lee, K. P. and Rozenberg, G.},
     TITLE = {Subword complexities of various classes of deterministic
              developmental languages with interactions},
   JOURNAL = {Internat. J. Comput. Information Sci.},
  FJOURNAL = {International Journal of Computer and Information Sciences},
    VOLUME = {4},
      YEAR = {1975},
    NUMBER = {3},
     PAGES = {219--236},
      ISSN = {0091-7036},
   MRCLASS = {68A30 (92A10)},
  MRNUMBER = {0433997 (55 \#6967)},
MRREVIEWER = {Branislav Rovan},
}

@article {EhrRoz82,
    AUTHOR = {Ehrenfeucht, A. and Rozenberg, G.},
     TITLE = {On subword complexities of homomorphic images of languages},
   JOURNAL = {RAIRO Inform. Th\'eor.},
  FJOURNAL = {RAIRO Informatique Th\'eorique},
    VOLUME = {16},
      YEAR = {1982},
    NUMBER = {4},
     PAGES = {303--316},
      ISSN = {0399-0540},
     CODEN = {RSITD7},
   MRCLASS = {68F05},
  MRNUMBER = {707633 (84i:68126)},
}

@article {Ehr57,
    AUTHOR = {Ehresmann, C.},
     TITLE = {Gattungen von lokalen {S}trukturen},
   JOURNAL = {Jber. Deutsch. Math. Verein.},
  FJOURNAL = {Jahresbericht der Deutschen Mathematiker-Vereinigung},
    VOLUME = {60},
      YEAR = {1957},
    NUMBER = {Abt. 1},
     PAGES = {49--77},
      ISSN = {0012-0456},
   MRCLASS = {20.00 (08.00)},
  MRNUMBER = {0095894 (20 \#2392)},
MRREVIEWER = {H. Samelson},
}

@article {Ell82,
    AUTHOR = {Elliott, G. A.},
     TITLE = {Gaps in the spectrum of an almost periodic {S}chr\"o\-dinger
              operator},
   JOURNAL = {C. R. Math. Rep. Acad. Sci. Canada},
  FJOURNAL = {La Soci\'et\'e Royale du Canada. L'Academie des Sciences.
              Comptes Rendus Math\'ematiques. (Mathematical Reports)},
    VOLUME = {4},
      YEAR = {1982},
    NUMBER = {5},
     PAGES = {255--259},
      ISSN = {0706-1994},
   MRCLASS = {47E05 (34B25 46L99 58F11)},
  MRNUMBER = {675127 (85b:47054)},
MRREVIEWER = {Fumio Hiai},
}

@article {Els85a,
    title = {Indexing problems in quasicrystal diffraction},
   author = {Elser, V.},
  journal = {Phys. Rev. B},
   volume = {32},
    issue = {8},
    pages = {4892--4898},
     year = {1985},
    month = {Oct},
publisher = {American Physical Society},
      doi = {10.1103/PhysRevB.32.4892},
      url = {http://link.aps.org/doi/10.1103/PhysRevB.32.4892},
}


@article {Els85b,
    title = {Comment on "Quasicrystals: A New Class of Ordered Structures"},
   author = {Elser, V.},
  journal = {Phys. Rev. Lett.},
   volume = {54},
    issue = {15},
    pages = {1730--1730},
     year = {1985},
    month = {Apr},
publisher = {American Physical Society},
      doi = {10.1103/PhysRevLett.54.1730},
      url = {http://link.aps.org/doi/10.1103/PhysRevLett.54.1730},
}


@incollection {Exe14,
    AUTHOR = {Exel, R.},
     TITLE = {Invertibility in groupoid {${C}^{\ast}$}-algebras},
 BOOKTITLE = {Operator theory, opera\-tor algebras and applications},
    SERIES = {Oper. Theory Adv. Appl.},
    VOLUME = {242},
     PAGES = {173--183},
 PUBLISHER = {Birk\-h\"auser/Springer, Basel},
      YEAR = {2014},
   MRCLASS = {22A22 (46L05)},
  MRNUMBER = {3243289},
       DOI = {10.1007/978-3-0348-0816-3_9},
       URL = {http://dx.doi.org/10.1007/978-3-0348-0816-3_9},
}

@article {FaLiWe11,
    AUTHOR = {Fan, S. and Liu, Q.-H. and Wen, Z.-Y.},
     TITLE = {Gibbs-like measure for spectrum of a class of quasi-crystals},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {31},
      YEAR = {2011},
    NUMBER = {6},
     PAGES = {1669--1695},
      ISSN = {0143-3857},
   MRCLASS = {37A30 (28A80 39A70 52C23)},
  MRNUMBER = {2851671},
MRREVIEWER = {Juan Garc{\'{\i}}a Escudero},
       DOI = {10.1017/S0143385710000635},
       URL = {http://dx.doi.org/10.1017/S0143385710000635},
}

@article {Fav28,
    AUTHOR = {Favard, J.},
     TITLE = {Sur les \'equations diff\'erentielles lin\'eaires \`a
              coefficients presque-p\'eriodiques},
   JOURNAL = {Acta Math.},
  FJOURNAL = {Acta Mathematica},
    VOLUME = {51},
      YEAR = {1928},
    NUMBER = {1},
     PAGES = {31--81},
      ISSN = {0001-5962},
     CODEN = {ACMAA8},
   MRCLASS = {Contributed Item},
  MRNUMBER = {1555261},
       DOI = {10.1007/BF02545660},
       URL = {http://dx.doi.org/10.1007/BF02545660},
}

@article {FeZe99,
    AUTHOR = {Feinberg, J. and Zee, A.},
     TITLE = {Spectral curves of non-{H}ermitian {H}amiltonians},
   JOURNAL = {Nuclear Phys. B},
  FJOURNAL = {Nuclear Physics. B},
    VOLUME = {552},
      YEAR = {1999},
    NUMBER = {3},
     PAGES = {599--623},
      ISSN = {0550-3213},
     CODEN = {NUPBBO},
   MRCLASS = {82B44 (82D55)},
  MRNUMBER = {1704620 (2000c:82044)},
       DOI = {10.1016/S0550-3213(99)00246-1},
       URL = {http://dx.doi.org/10.1016/S0550-3213(99)00246-1},
}

@article {Fel60,
    AUTHOR = {Fell, J. M. G.},
     TITLE = {The dual spaces of {$C^{\ast} $}-algebras},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {94},
      YEAR = {1960},
     PAGES = {365--403},
      ISSN = {0002-9947},
   MRCLASS = {46.65},
  MRNUMBER = {0146681},
MRREVIEWER = {R. Arens},
}

@article {Fel61,
    AUTHOR = {Fell, J. M. G.},
     TITLE = {The structure of algebras of operator fields},
   JOURNAL = {Acta Math.},
  FJOURNAL = {Acta Mathematica},
    VOLUME = {106},
      YEAR = {1961},
     PAGES = {233--280},
      ISSN = {0001-5962},
   MRCLASS = {46.65},
  MRNUMBER = {0164248 (29 \#1547)},
MRREVIEWER = {B. Yood},
}

@article {Fel62,
    AUTHOR = {Fell, J. M. G.},
     TITLE = {A {H}ausdorff topology for the closed subsets of a locally
              compact non-{H}ausdorff space},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {13},
      YEAR = {1962},
     PAGES = {472--476},
      ISSN = {0002-9939},
   MRCLASS = {54.52 (54.53)},
  MRNUMBER = {0139135 (25 \#2573)},
MRREVIEWER = {F. Cunningham, Jr.},
}

@article {FeWeWu97,
    AUTHOR = {Feng, D. and Wen, Z. and Wu, J.},
     TITLE = {Some dimensional results for homogeneous {M}oran sets},
   JOURNAL = {Sci. China Ser. A},
  FJOURNAL = {Science in China. Series A. Mathematics},
    VOLUME = {40},
      YEAR = {1997},
    NUMBER = {5},
     PAGES = {475--482},
      ISSN = {1006-9283},
   MRCLASS = {28A78 (28A80)},
  MRNUMBER = {1461002},
       DOI = {10.1007/BF02896955},
       URL = {http://dx.doi.org/10.1007/BF02896955},
}

@article {Fer95,
    AUTHOR = {Ferenczi, S.},
     TITLE = {Les transformations de {C}hacon: combinatoire, structure
              g\'{e}o\-m\'{e}trique, lien avec les syst\`emes de complexit\'e
              {$2n+1$}},
   JOURNAL = {Bull. Soc. Math. France},
  FJOURNAL = {Bulletin de la Soci\'et\'e Math\'ematique de France},
    VOLUME = {123},
      YEAR = {1995},
    NUMBER = {2},
     PAGES = {271--292},
      ISSN = {0037-9484},
     CODEN = {BSMFAA},
   MRCLASS = {28D05 (68R15)},
  MRNUMBER = {1340291},
MRREVIEWER = {Pierre Michel},
       URL = {http://www.numdam.org/item?id=BSMF_1995__123_2_271_0},
}

@book {Fil98,
    AUTHOR = {Filippov, V. V.},
     TITLE = {Basic topological structures of ordinary differential
              equations},
    SERIES = {Mathematics and its Applications},
    VOLUME = {432},
      NOTE = {Translated from the Russian},
 PUBLISHER = {Kluwer Academic Publishers, Dordrecht},
      YEAR = {1998},
     PAGES = {xiv+516},
      ISBN = {0-7923-4951-2},
   MRCLASS = {34-02 (34A12 34A36 34A60 34Cxx 54-02)},
  MRNUMBER = {1651066 (2000c:34001)},
MRREVIEWER = {Zvi Artstein},
       DOI = {10.1007/978-94-017-0841-8},
       URL = {http://dx.doi.org/10.1007/978-94-017-0841-8},
}

@article {Fio09,
    AUTHOR = {Fiorenzi, F.},
     TITLE = {Periodic configurations of subshifts on groups},
   JOURNAL = {Internat. J. Algebra Comput.},
  FJOURNAL = {International Journal of Algebra and Computation},
    VOLUME = {19},
      YEAR = {2009},
    NUMBER = {3},
     PAGES = {315--335},
      ISSN = {0218-1967},
   MRCLASS = {37B10 (68Q80)},
  MRNUMBER = {2522838 (2010m:37016)},
MRREVIEWER = {Michael Hurley},
       DOI = {10.1142/S0218196709005123},
       URL = {http://dx.doi.org/10.1142/S0218196709005123},
}

@article {Flo1883,
    AUTHOR = {Floquet, G.},
     TITLE = {Sur les \'equations diff\'erentielles lin\'eaires \`a
              coefficients p\'erio\-diques},
   JOURNAL = {Ann. Sci. \'Ecole Norm. Sup. (2)},
  FJOURNAL = {Annales Scientifiques de l'\'Ecole Normale Sup\'erieure.
              Deuxi\'eme S\'erie},
    VOLUME = {12},
      YEAR = {1883},
     PAGES = {47--88},
      ISSN = {0012-9593},
   MRCLASS = {Contributed Item},
  MRNUMBER = {1508722},
       URL = {http://www.numdam.org/item?id=ASENS_1883_2_12__47_0},
}

@article {Fly1894,
    AUTHOR = {Flye Sainte-Marie, C.},
     TITLE = {Question 48},
   JOURNAL = {L'Interm\'{e}diaire Math.},
  FJOURNAL = {L'Interm\'{e}diaire des math\'{e}maticiens},
    VOLUME = {1},
      YEAR = {1894},
     PAGES = {107--110},
}

@article {Fra05,
    AUTHOR = {Frank, N. P.},
     TITLE = {Multidimensional constant-length substitution sequences},
   JOURNAL = {Topology Appl.},
  FJOURNAL = {Topology and its Applications},
    VOLUME = {152},
      YEAR = {2005},
    NUMBER = {1-2},
     PAGES = {44--69},
      ISSN = {0166-8641},
     CODEN = {TIAPD9},
   MRCLASS = {37B50 (37A30 37B10)},
  MRNUMBER = {2160805},
MRREVIEWER = {Reem Yassawi},
       DOI = {10.1016/j.topol.2004.08.014},
       URL = {http://dx.doi.org/10.1016/j.topol.2004.08.014},
}

@article {Fra08,
    AUTHOR = {Frank, N. P.},
     TITLE = {A primer of substitution tilings of the {E}uclidean plane},
   JOURNAL = {Expo. Math.},
  FJOURNAL = {Expositiones Mathematicae},
    VOLUME = {26},
      YEAR = {2008},
    NUMBER = {4},
     PAGES = {295--326},
      ISSN = {0723-0869},
   MRCLASS = {52C23 (37B50 52C20)},
  MRNUMBER = {2462439},
MRREVIEWER = {Ana Maria d'Azevedo Breda},
       DOI = {10.1016/j.exmath.2008.02.001},
       URL = {http://dx.doi.org/10.1016/j.exmath.2008.02.001},
}

@misc {FrSp83,
    AUTHOR = {Fr{\"o}hlich, J. and Spencer, T.},
     TITLE = {Absence of diffusion in the {A}nderson tight binding model for
              large disorder or low energy},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {88},
      YEAR = {1983},
    NUMBER = {2},
     PAGES = {151--184},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {82A05 (60H25 82A57)},
  MRNUMBER = {696803},
MRREVIEWER = {W. Kirsch},
       URL = {http://projecteuclid.org/euclid.cmp/1103922279},
}

@misc {FrMaScSp85,
    AUTHOR = {Fr{\"o}hlich, J. and Martinelli, F. and Scoppola, E. and Spencer, T.},
     TITLE = {Constructive proof of localization in the {A}nderson tight
              binding model},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {101},
      YEAR = {1985},
    NUMBER = {1},
     PAGES = {21--46},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {82A57 (60H25 81C10)},
  MRNUMBER = {814541},
MRREVIEWER = {Italo Guarneri},
       URL = {http://projecteuclid.org/euclid.cmp/1104114065},
}

@article {GaMa06,
    AUTHOR = {Gambaudo, J.-M. and Martens, M.},
     TITLE = {Algebraic topology for minimal {C}antor sets},
   JOURNAL = {Ann. Henri Poincar\'e},
  FJOURNAL = {Annales Henri Poincar\'e. A Journal of Theoretical and
              Mathematical Physics},
    VOLUME = {7},
      YEAR = {2006},
    NUMBER = {3},
     PAGES = {423--446},
      ISSN = {1424-0637},
   MRCLASS = {37B05 (37A25 37B40 55P99)},
  MRNUMBER = {2226743},
MRREVIEWER = {Fred W. Roush},
       DOI = {10.1007/s00023-005-0255-3},
       URL = {http://dx.doi.org/10.1007/s00023-005-0255-3},
}

@misc {Gah02,
    AUTHOR = {G{\"a}hler, F.},
     TITLE = {Periodic configurations of subshifts on groups},
      YEAR = {August 4-8,2002},
      Note = {talk given at the conference {A}periodic O{}rder, {D}ynamical {S}ystems, {O}perator {A}lgebra and {T}opology, Victoria, B.C., Canada. (unpublished)},
}

@misc {GaHuKe05,
    AUTHOR = {G{\"a}hler, F. and Hunton, J. R. and Kellendonk, J.},
     TITLE = {Torsion in Tiling Homology and Cohomology},
      NOTE = {arXiv:math-ph/0505048},
      YEAR = {2005},
       URL = {http://arxiv.org/abs/math-ph/0505048},
}

@misc {GaHuKe08,
    AUTHOR = {G{\"a}hler, F. and Hunton, J. R. and Kellendonk, J.},
     TITLE = {Integer Cech Cohomology of Icosahedral Projection Tilings},
      NOTE = {arXiv:0809.4442},
      YEAR = {2008},
       URL = {http://arxiv.org/abs/0809.4442},
}

@preamble{
   "\def\cprime{$'$} "
}
@incollection {GeNe43,
    AUTHOR = {Gel{\cprime}fand, I. and Neumark, M.},
     TITLE = {On the imbedding of normed rings into the ring of operators in
              {H}ilbert space},
 BOOKTITLE = {{${C}^{\ast}$}-algebras: 1943--1993 ({S}an {A}ntonio, {TX},
              1993)},
    SERIES = {Contemp. Math.},
    VOLUME = {167},
     PAGES = {2--19},
      NOTE = {Corrected reprint of the 1943 original [MR {{\bf{5}}}, 147]},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {1994},
   MRCLASS = {46L05 (01A75)},
  MRNUMBER = {1292007},
       DOI = {10.1090/conm/167/1292007},
       URL = {http://dx.doi.org/10.1090/conm/167/1292007},
}

@misc {GrLeNa14,
    AUTHOR = {Grigorchuk, R. and Lenz, D. and Nagnibeda, T.},
     TITLE = {{S}pectra of {S}chreier graphs of {G}rigorchuk's group and {S}chr{\"o}dinger operators with aperiodic order},
      NOTE = {arXiv:1412.6822},
      YEAR = {2014},
       URL = {http://arxiv.org/abs/1412.6822},
}

@misc {GrLeNa15,
    AUTHOR = {Grigorchuk, R. and Lenz, D. and Nagnibeda, T.},
     TITLE = {{S}chreier graphs of {G}rigorchuk's group and a subshift associated to a non-primitive substitution},
      NOTE = {arXiv:1510.00545},
      YEAR = {2015},
       URL = {http://arxiv.org/abs/1510.00545},
}

@article {Gol49,
    AUTHOR = {Golay, M. J. L.},
     TITLE = {{M}ulti-slit spectrometry},
   JOURNAL = {J. Optical Soc. America},
  FJOURNAL = {Journal of the Optical Society of America},
    VOLUME = {39},
    NUMBER = {6},
      YEAR = {1949},
     PAGES = {137--444},
       DOI = {10.1364/JOSA.39.000437},
}

@article {GoMoPa77,
    AUTHOR = {Goldsheid, I. Ya. and Molchanov, S. A. and Pastur, L. A.},
     TITLE = {A random homogeneous {S}chr{\"o}dinger operator has a pure point spectrum},
   JOURNAL = {(Russian) Funkcional. Anal. i Prilo{\`z}en.},
    VOLUME = {11},
    NUMBER = {96},
      YEAR = {1977},
     PAGES = {1--10},
}

@article {Goo46,
    AUTHOR = {Good, I. J.},
     TITLE = {Normal recurring decimals},
   JOURNAL = {J. London Math. Soc.},
  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {21},
      YEAR = {1946},
     PAGES = {167--169},
      ISSN = {0024-6107},
   MRCLASS = {09.0X},
  MRNUMBER = {0019573 (8,430k)},
MRREVIEWER = {P. Erd{\"o}s},
}

@article {GrOrRo15,
    AUTHOR = {Gr{\"o}chenig, K. and Ortega-Cerd{\`a}, J. and
              Romero, J. L.},
     TITLE = {Deformation of {G}abor systems},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {277},
      YEAR = {2015},
     PAGES = {388--425},
      ISSN = {0001-8708},
   MRCLASS = {42C15 (47B38 81R30 94A12)},
  MRNUMBER = {3336091},
MRREVIEWER = {Ilona Iglewska-Nowak},
       DOI = {10.1016/j.aim.2015.01.019},
       URL = {http://dx.doi.org/10.1016/j.aim.2015.01.019},
}

@article {Hah78,
    AUTHOR = {Hahn, P.},
     TITLE = {The regular representations of measure groupoids},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {242},
      YEAR = {1978},
     PAGES = {35--72},
      ISSN = {0002-9947},
     CODEN = {TAMTAM},
   MRCLASS = {46L10 (28D99 46K15)},
  MRNUMBER = {496797 (81f:46075)},
       DOI = {10.2307/1997727},
       URL = {http://dx.doi.org/10.2307/1997727},
}

@article {HaWa01,
    AUTHOR = {Hajduk, B. and Walczak, R.},
     TITLE = {Invariant metrics on {$G$}-spaces},
   JOURNAL = {Czechoslovak Math. J.},
  FJOURNAL = {Czechoslovak Mathematical Journal},
    VOLUME = {53(128)},
      YEAR = {2003},
    NUMBER = {2},
     PAGES = {449--466},
      ISSN = {0011-4642},
     CODEN = {CZMJAE},
   MRCLASS = {54H15 (54E35)},
  MRNUMBER = {1983465},
MRREVIEWER = {Helmut Ludescher},
       DOI = {10.1023/A:1026251807392},
       URL = {http://dx.doi.org/10.1023/A:1026251807392},
}

@article{Har55,
  author={Harper, P. G.},
  title={Single Band Motion of Conduction Electrons in a Uniform Magnetic Field},
  journal={Proceedings of the Physical Society. Section A},
  volume={68},
  number={10},
  pages={874},
  url={http://stacks.iop.org/0370-1298/68/i=10/a=304},
  year={1955},
  abstract={The effect of a uniform magnetic field on the conduction band of metal is investigated, using as model the tight-binding approximation for a simple cubic crystal. The normally discrete magnetic levels pertaining to free electrons are shown to be non-uniformly spaced and broadened as a result of the lattice forces.}
}

@article{HaNe96,
  author = {Hatano, N. and Nelson, D. R.},
  title = {Localization Transitions in Non-Hermitian Quantum Mechanics},
  journal = {Phys. Rev. Lett.},
  volume = {77},
  issue = {3},
  pages = {570--573},
  year = {1996},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.77.570},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.77.570}
}

@misc {HaKoWa15,
    AUTHOR = {Haynes, A. and Koivusalo, H. and Walton, J.},
     TITLE = {A characterization of linearly repetitive cut and project sets},
      NOTE = {arXiv:1503.04091},
      YEAR = {2015},
       URL = {http://arxiv.org/abs/1503.04091},
}

@article {Hay16,
    AUTHOR = {Haynes, A.},
     TITLE = {Equivalence classes of codimension-one cut-and-project nets},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {36},
      YEAR = {2016},
    NUMBER = {3},
     PAGES = {816--831},
      ISSN = {0143-3857},
   MRCLASS = {26B35 (26B12)},
  MRNUMBER = {3480345},
       DOI = {10.1017/etds.2014.90},
       URL = {http://dx.doi.org/10.1017/etds.2014.90},
}

@article {HaKo16,
    AUTHOR = {Haynes, A. and Koivusalo, H.},
     TITLE = {Constructing bounded remainder sets and cut-and-project sets
              which are bounded distance to lattices},
   JOURNAL = {Israel J. Math.},
  FJOURNAL = {Israel Journal of Mathematics},
    VOLUME = {212},
      YEAR = {2016},
    NUMBER = {1},
     PAGES = {189--201},
      ISSN = {0021-2172},
   MRCLASS = {Preliminary Data},
  MRNUMBER = {3504323},
       DOI = {10.1007/s11856-016-1283-z},
       URL = {http://dx.doi.org/10.1007/s11856-016-1283-z},
}

@article {HaKoSaWa16,
    AUTHOR = {Haynes, A. and Koivusalo, H. and Sadun, L. and Walton, J.},
     TITLE = {Gaps problems and frequencies of patches in cut and project
              sets},
   JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
  FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
              Society},
    VOLUME = {161},
      YEAR = {2016},
    NUMBER = {1},
     PAGES = {65--85},
      ISSN = {0305-0041},
   MRCLASS = {Preliminary Data},
  MRNUMBER = {3505670},
       DOI = {10.1017/S0305004116000128},
       URL = {http://dx.doi.org/10.1017/S0305004116000128},
}

@article {HeSj87,
    AUTHOR = {Helffer, B. and Sj{\"o}strand, J.},
   JOURNAL = {Ann. Scuola Norm. Sup. Pisa Cl. Sci.},
  fjournal = {Annali della Scuola Normale Superiore di Pisa - Classe di Scienze},
    number = {4},
     pages = {625-657},
 publisher = {Scuola normale superiore},
     title = {Effet tunnel pour l'{\'{e}}quation de {}chrödinger avec champ magn{\'{e}}tique},
       url = {http://eudml.org/doc/84021},
    volume = {14},
      year = {1987},
}

@article {HeSj89,
    AUTHOR = {Helffer, B. and Sj{\"o}strand, J.},
     TITLE = {Analyse semi-classique pour l’{\'{e}}quation de {H}arper },
   JOURNAL = {Mem. Soc. Math. France (N.S.)},
  FJOURNAL = {Recherche Coopérative sur Programme n°25},
     pages = {1-18},
 publisher = {Institut de Recherche Math{\'{e}}matique Avancée - Universit{\'{e}} Louis Pasteur},
       url = {http://eudml.org/doc/274889},
    volume = {40},
      year = {1989},
}

@article {HeSj90,
    AUTHOR = {Helffer, B. and Sj{\"o}strand, J.},
     TITLE = {Analyse semi-classique pour l'{\'{e}}quation de {H}arper. {II}.\
              {C}omportement semi-classique pr{\'{e}}s d'un rationnel},
   JOURNAL = {M{\'{e}}m. Soc. Math. France (N.S.)},
  FJOURNAL = {M{\'{e}}moires de la Soci{\'{e}}t{\'{e}} Math{\'{e}}matique de France.
              Nouvelle S\'erie},
    NUMBER = {40},
      YEAR = {1990},
     PAGES = {139},
      ISSN = {0037-9484},
   MRCLASS = {35A27 (58G15 81Q15)},
  MRNUMBER = {1052373 (91h:35018)},
MRREVIEWER = {R{\'e}mi Vaillancourt},
}

@article {Her00,
    AUTHOR = {Hermisson, J.},
     TITLE = {Aperiodic and correlated disorder in {$XY$} chains: exact
              results},
   JOURNAL = {J. Phys. A},
  FJOURNAL = {Journal of Physics. A. Mathematical and General},
    VOLUME = {33},
      YEAR = {2000},
    NUMBER = {1},
     PAGES = {57--79},
      ISSN = {0305-4470},
     CODEN = {JPHAC5},
   MRCLASS = {82B44 (82B20)},
  MRNUMBER = {1748463 (2001a:82040)},
       DOI = {10.1088/0305-4470/33/1/304},
       URL = {http://dx.doi.org/10.1088/0305-4470/33/1/304},
}

@article {HiSk87,
    AUTHOR = {Hilsum, M. and Skandalis, G.},
     TITLE = {Morphismes {$K$}-orient\'es d'espaces de feuilles et
              fonctorialit\'e en th\'eorie de {K}asparov (d'apr\`es une
              conjecture d'{A}. {C}onnes)},
   JOURNAL = {Ann. Sci. \'Ecole Norm. Sup. (4)},
  FJOURNAL = {Annales Scientifiques de l'\'Ecole Normale Sup\'erieure.
              Quatri\`eme S\'erie},
    VOLUME = {20},
      YEAR = {1987},
    NUMBER = {3},
     PAGES = {325--390},
      ISSN = {0012-9593},
     CODEN = {ASENAH},
   MRCLASS = {58G12 (19K56 46L80 46M20 57R30 57R32 58G15)},
  MRNUMBER = {925720},
MRREVIEWER = {Jonathan M. Rosenberg},
       URL = {http://www.numdam.org/item?id=ASENS_1987_4_20_3_325_0},
}

@misc{Hoc09,
  author = {Hochman, M.},
   title = {Are the periodic points dense in multidimensional strongly irreducible {SFT}s?},
    year = {2009},
howpublished = {\! http://math.huji.ac.il/$\sim$mhochman/problems/periodic-points-of-SFTs.pdf},
    note = {online accessed March 16, 2016}
}

@article {HoKnSi95,
    AUTHOR = {Hof, A. and Knill, O. and Simon, B.},
     TITLE = {Singular continuous spectrum for palindromic {S}chr\"odinger
              operators},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {174},
      YEAR = {1995},
    NUMBER = {1},
     PAGES = {149--159},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {47B39 (47N50 81Q10)},
  MRNUMBER = {1372804},
MRREVIEWER = {Fr{\'e}d{\'e}ric Klopp},
       URL = {http://projecteuclid.org/euclid.cmp/1104275098},
}

@article{Hof76,
  author = {Hofstadter, D. R.},
  title = {Energy levels and wave functions of {B}loch electrons in rational and irrational magnetic fields},
  journal = {Phys. Rev. B},
  volume = {14},
  issue = {6},
  pages = {2239--2249},
  numpages = {0},
  year = {1976},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.14.2239},
  url = {http://link.aps.org/doi/10.1103/PhysRevB.14.2239}
}

@article {HuRaWeWu00,
    AUTHOR = {Hua, S. and Rao, H. and Wen, Z. and Wu, J.},
     TITLE = {On the structures and dimensions of {M}oran sets},
   JOURNAL = {Sci. China Ser. A},
  FJOURNAL = {Science in China. Series A. Mathematics},
    VOLUME = {43},
      YEAR = {2000},
    NUMBER = {8},
     PAGES = {836--852},
      ISSN = {1006-9283},
   MRCLASS = {28A78 (28A80)},
  MRNUMBER = {1799919},
MRREVIEWER = {Manuel Mor{\'a}n},
       DOI = {10.1007/BF02884183},
       URL = {http://dx.doi.org/10.1007/BF02884183},
}

@article {Hul66,
    AUTHOR = {Hulanicki, A.},
     TITLE = {Means and {F}\o lner condition on locally compact groups},
   JOURNAL = {Studia Math.},
  FJOURNAL = {Polska Akademia Nauk. Instytut Matematyczny. Studia
              Mathematica},
    VOLUME = {27},
      YEAR = {1966},
     PAGES = {87--104},
      ISSN = {0039-3223},
   MRCLASS = {22.65 (42.50)},
  MRNUMBER = {0195982 (33 \#4178)},
MRREVIEWER = {M. M. Day},
}

@incollection {Jit95,
    AUTHOR = {Jitomirskaya, S. Y.},
     TITLE = {Almost everything about the almost {M}athieu operator. {II}},
 BOOKTITLE = {X{I}th {I}nternational {C}ongress of {M}athematical {P}hysics
              ({P}aris, 1994)},
     PAGES = {373--382},
 PUBLISHER = {Int. Press, Cambridge, MA},
      YEAR = {1995},
   MRCLASS = {82B44 (39A70 47B39 47B50 81Q10 81Q50)},
  MRNUMBER = {1370694 (96m:82035)},
MRREVIEWER = {Nariyuki Minami},
}

@article {JiKr02,
    AUTHOR = {Jitomirskaya, S. Y. and Krasovsky, I. V.},
     TITLE = {Continuity of the measure of the spectrum for discrete
              quasiperiodic operators},
   JOURNAL = {Math. Res. Lett.},
  FJOURNAL = {Mathematical Research Letters},
    VOLUME = {9},
      YEAR = {2002},
    NUMBER = {4},
     PAGES = {413--421},
      ISSN = {1073-2780},
   MRCLASS = {81Q10 (39A12 39A70 82B44)},
  MRNUMBER = {1928861 (2004b:81051)},
MRREVIEWER = {Kalyan B. Sinha},
       DOI = {10.4310/MRL.2002.v9.n4.a1},
       URL = {http://dx.doi.org/10.4310/MRL.2002.v9.n4.a1},
}
	

@article {Jul10,
    AUTHOR = {Julien, A.},
     TITLE = {Complexity and cohomology for cut-and-projection tilings},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {30},
      YEAR = {2010},
    NUMBER = {2},
     PAGES = {489--523},
      ISSN = {0143-3857},
   MRCLASS = {52C45 (05B45 37B50 52C23)},
  MRNUMBER = {2599890 (2011i:52045)},
MRREVIEWER = {Bernd Sing},
       DOI = {10.1017/S0143385709000194},
       URL = {http://dx.doi.org/10.1017/S0143385709000194},
}

@article {Joh86,
    AUTHOR = {Johnson, R. A.},
     TITLE = {Exponential dichotomy, rotation number, and linear
              differential operators with bounded coefficients},
   JOURNAL = {J. Differential Equations},
  FJOURNAL = {Journal of Differential Equations},
    VOLUME = {61},
      YEAR = {1986},
    NUMBER = {1},
     PAGES = {54--78},
      ISSN = {0022-0396},
     CODEN = {JDEQAK},
   MRCLASS = {47E05 (34A20 47B39 58F19)},
  MRNUMBER = {818861 (87e:47065)},
MRREVIEWER = {A. Pelczar},
       DOI = {10.1016/0022-0396(86)90125-7},
       URL = {http://dx.doi.org/10.1016/0022-0396(86)90125-7},
}

@article {KaKiLe85a,
   author = {{Kalugin}, P.~A. and {Kitaev}, A.~I. and {Levitov}, L.~S.},
    title = {Al(0.86)Mn(0.14) - A six-dimensional crystal},
  journal = {ZhETF Pisma Redaktsiiu},
     year = {1985},
    month = {feb},
   volume = {41},
    pages = {119--121},
   adsurl = {http://adsabs.harvard.edu/abs/1985ZhPmR..41..119K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article {KaKiLe85b,
    AUTHOR = {Kalugin, P. A. and Kitaev, A.Y. and Levitov, L. S.},
     TITLE = {6-dimensional properties of Al(0.86)Mn(0.14)},
   JOURNAL = {J. Physique Lett. (France)},
     PAGES = {601--607},
    VOLUME = {46},
    NUMBER = {13},
      YEAR = {1985},
       DOI = {10.1051/jphyslet:019850046013060100},
}

@article {KaPu03,
    AUTHOR = {Kaminker, J. and Putnam, I.},
     TITLE = {A proof of the gap labeling conjecture},
   JOURNAL = {Michigan Math. J.},
  FJOURNAL = {The Michigan Mathematical Journal},
    VOLUME = {51},
      YEAR = {2003},
    NUMBER = {3},
     PAGES = {537--546},
      ISSN = {0026-2285},
   MRCLASS = {46L55 (19K14 37B50 46L80 46N50 52C23)},
  MRNUMBER = {2021006},
MRREVIEWER = {Claude Schochet},
}

@article {Kap49,
    AUTHOR = {Kaplansky, I.},
     TITLE = {Normed algebras},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {16},
      YEAR = {1949},
     PAGES = {399--418},
      ISSN = {0012-7094},
   MRCLASS = {46.3X},
  MRNUMBER = {0031193},
MRREVIEWER = {R. Godement},
}

@article {Kap51,
    AUTHOR = {Kaplansky, I.},
     TITLE = {The structure of certain operator algebras},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {70},
      YEAR = {1951},
     PAGES = {219--255},
      ISSN = {0002-9947},
   MRCLASS = {46.3X},
  MRNUMBER = {0042066 (13,48a)},
MRREVIEWER = {R. Godement},
}

@article {Kel95,
    AUTHOR = {Kellendonk, J.},
     TITLE = {Noncommutative geometry of tilings and gap labelling},
   JOURNAL = {Rev. Math. Phys.},
  FJOURNAL = {Reviews in Mathematical Physics. A Journal for Both Review and
              Original Research Papers in the Field of Mathematical Physics},
    VOLUME = {7},
      YEAR = {1995},
    NUMBER = {7},
     PAGES = {1133--1180},
      ISSN = {0129-055X},
   MRCLASS = {46L87 (05B45 19K14 46L55 46L80 52C20 52C22 82D25)},
  MRNUMBER = {1359991},
MRREVIEWER = {Albert Jeu-Liang Sheu},
       DOI = {10.1142/S0129055X95000426},
       URL = {http://dx.doi.org/10.1142/S0129055X95000426},
}

@article {Kel97,
    AUTHOR = {Kellendonk, J.},
     TITLE = {The local structure of tilings and their integer group of
              coinvariants},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {187},
      YEAR = {1997},
    NUMBER = {1},
     PAGES = {115--157},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {46L87 (52C22)},
  MRNUMBER = {1463824 (98m:46090)},
MRREVIEWER = {G. A. Noskov},
       DOI = {10.1007/s002200050131},
       URL = {http://dx.doi.org/10.1007/s002200050131},
}

@incollection {KePu00,
    AUTHOR = {Kellendonk, J. and Putnam, I. F.},
     TITLE = {Tilings, {${C}^{\ast}$}-algebras, and {$K$}-theory},
 BOOKTITLE = {Directions in mathematical quasicrystals},
    SERIES = {CRM Monogr. Ser.},
    VOLUME = {13},
     PAGES = {177--206},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2000},
   MRCLASS = {46L60 (19K14 37B50 46L80 52C23 82D25)},
  MRNUMBER = {1798993 (2001m:46153)},
MRREVIEWER = {G. A. Noskov},
}

@article {Kel03,
    AUTHOR = {Kellendonk, J.},
     TITLE = {Pattern-equivariant functions and cohomology},
   JOURNAL = {J. Phys. A},
  FJOURNAL = {Journal of Physics. A. Mathematical and General},
    VOLUME = {36},
      YEAR = {2003},
    NUMBER = {21},
     PAGES = {5765--5772},
      ISSN = {0305-4470},
     CODEN = {JPHAC5},
   MRCLASS = {52C23},
  MRNUMBER = {1985494 (2004e:52025)},
       DOI = {10.1088/0305-4470/36/21/306},
       URL = {http://dx.doi.org/10.1088/0305-4470/36/21/306},
}

@article {KoKaTa83,
    AUTHOR = {Kohmoto, M. and Kadanoff, L. P. and Tang, C.},
     TITLE = {Localization problem in one dimension: mapping and escape},
   JOURNAL = {Phys. Rev. Lett.},
  FJOURNAL = {Physical Review Letters},
    VOLUME = {50},
      YEAR = {1983},
    NUMBER = {23},
     PAGES = {1870--1872},
      ISSN = {0031-9007},
     CODEN = {PRLTAO},
   MRCLASS = {58F27 (81C05 82A05 82A55)},
  MRNUMBER = {702474},
MRREVIEWER = {Helmut R{\"u}ssmann},
       DOI = {10.1103/PhysRevLett.50.1870},
       URL = {http://dx.doi.org/10.1103/PhysRevLett.50.1870},
}

@article {Kol53,
    AUTHOR = {Kolmogorov, A. N.},
     TITLE = {On dynamical systems with an integral invariant on the torus},
   JOURNAL = {Doklady Akad. Nauk SSSR (N.S.)},
    VOLUME = {93},
      YEAR = {1953},
     PAGES = {763--766},
   MRCLASS = {36.0X},
  MRNUMBER = {0062892},
MRREVIEWER = {Y. N. Dowker},
}

@article {Kol54,
    AUTHOR = {Kolmogorov, A. N.},
     TITLE = {On conservation of conditionally periodic motions for a small
              change in {H}amilton's function},
   JOURNAL = {Dokl. Akad. Nauk SSSR (N.S.)},
  FJOURNAL = {Doklady Akademii Nauk SSSR},
    VOLUME = {98},
      YEAR = {1954},
     PAGES = {527--530},
      ISSN = {0002-3264},
   MRCLASS = {36.0X},
  MRNUMBER = {0068687},
MRREVIEWER = {Y. N. Dowker},
}

@article {Kot89,
    AUTHOR = {Kotani, S.},
     TITLE = {Jacobi matrices with random potentials taking finitely many
              values},
   JOURNAL = {Rev. Math. Phys.},
  FJOURNAL = {Reviews in Mathematical Physics. A Journal for Both Review and
              Original Research Papers in the Field of Mathematical Physics},
    VOLUME = {1},
      YEAR = {1989},
    NUMBER = {1},
     PAGES = {129--133},
      ISSN = {0129-055X},
   MRCLASS = {81Q10 (47B99 82B44)},
  MRNUMBER = {1041533 (91b:81023)},
MRREVIEWER = {Dimitri Petritis},
       DOI = {10.1142/S0129055X89000067},
       URL = {http://dx.doi.org/10.1142/S0129055X89000067},
}

@article {Krei16,
    AUTHOR = {Kreisel, M.},
     TITLE = {Gabor frames for quasicrystals, {$K$}-theory, and twisted gap
              labeling},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {270},
      YEAR = {2016},
    NUMBER = {3},
     PAGES = {1001--1030},
      ISSN = {0022-1236},
   MRCLASS = {Preliminary Data},
  MRNUMBER = {3438328},
       DOI = {10.1016/j.jfa.2015.11.011},
       URL = {http://dx.doi.org/10.1016/j.jfa.2015.11.011},
}

@article {Lag99,
    AUTHOR = {Lagarias, J. C.},
     TITLE = {Geometric models for quasicrystals {I}. {D}elone sets of
              finite type},
   JOURNAL = {Discrete Comput. Geom.},
  FJOURNAL = {Discrete \& Computational Geometry. An International Journal
              of Mathematics and Computer Science},
    VOLUME = {21},
      YEAR = {1999},
    NUMBER = {2},
     PAGES = {161--191},
      ISSN = {0179-5376},
     CODEN = {DCGEER},
   MRCLASS = {52C22},
  MRNUMBER = {1668082 (99m:52029)},
       DOI = {10.1007/PL00009413},
       URL = {http://dx.doi.org/10.1007/PL00009413},
}

@article {LaPl03,
    AUTHOR = {Lagarias, J. C. and Pleasants, P. A. B.},
     TITLE = {Repetitive {D}elone sets and quasicrystals},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {23},
      YEAR = {2003},
    NUMBER = {3},
     PAGES = {831--867},
      ISSN = {0143-3857},
   MRCLASS = {52C23 (37A25 37B50)},
  MRNUMBER = {1992666},
MRREVIEWER = {David Damanik},
       DOI = {10.1017/S0143385702001566},
       URL = {http://dx.doi.org/10.1017/S0143385702001566},
}

@incollection {LaRa99,
    AUTHOR = {Landsman, N. P. and Ramazan, B.},
     TITLE = {Quantization of {P}oisson algebras associated to {L}ie
              algebroids},
 BOOKTITLE = {Groupoids in analysis, geometry, and physics ({B}oulder, {CO},
              1999)},
    SERIES = {Contemp. Math.},
    VOLUME = {282},
     PAGES = {159--192},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2001},
   MRCLASS = {46L65 (22A22 46L60)},
  MRNUMBER = {1855249 (2002g:46119)},
       DOI = {10.1090/conm/282/04685},
       URL = {http://dx.doi.org/10.1090/conm/282/04685},
}

@misc {Lan16,
    AUTHOR = {Landstad, M. B.},
     TITLE = {Private discussion},
      YEAR = {2016},
     MONTH = {January},
}

@article {Lan98,
    AUTHOR = {Lang, F. G.},
     TITLE = {Schreiben nach {M}ass. Zur {S}tichometrie in der antiken {L}iteratur},
   JOURNAL = {Novum Testamentum},
    VOLUME = {41},
     PAGES = {40--57},
      YEAR = {1999},
 PUBLISHER = {Brill},
    NUMBER = {1},
       URL = {http://www.jstor.org/stable/1561477},
      ISSN = {00481009},
}

@article {LaRa85,
    AUTHOR = {Lange, B. V. and Rabinovich, V. S.},
     TITLE = {Noethericity of multidimensional discrete convolution
              operators},
   JOURNAL = {Mat. Zametki},
  FJOURNAL = {Akademiya Nauk SSSR. Matematicheskie Zametki},
    VOLUME = {37},
      YEAR = {1985},
    NUMBER = {3},
     PAGES = {407--421, 462},
      ISSN = {0025-567X},
   MRCLASS = {47B38},
  MRNUMBER = {790430 (87b:47035)},
MRREVIEWER = {N. L. Vasilevski{\u\i}},
}

@incollection {Last95,
    AUTHOR = {Last, Y.},
     TITLE = {Almost everything about the almost {M}athieu operator. {I}},
 BOOKTITLE = {X{I}th {I}nternational {C}ongress of {M}athematical {P}hysics
              ({P}aris, 1994)},
     PAGES = {366--372},
 PUBLISHER = {Int. Press, Cambridge, MA},
      YEAR = {1995},
   MRCLASS = {82B44 (39A70 47B39 47B50 81Q10 81Q50)},
  MRNUMBER = {1370693 (96m:82034)},
MRREVIEWER = {Nariyuki Minami},
}

@article {LaSi06,
    AUTHOR = {Last, Y. and Simon, B.},
     TITLE = {The essential spectrum of {S}chr\"odinger, {J}acobi, and {CMV} operators},
   JOURNAL = {J. Anal. Math.},
  FJOURNAL = {Journal d'Analyse Math\'ematique},
    VOLUME = {98},
      YEAR = {2006},
     PAGES = {183--220},
      ISSN = {0021-7670},
     CODEN = {JOAMAV},
   MRCLASS = {47A10 (34L40 35P05 47B36 47E05 47F05 81Q10)},
  MRNUMBER = {2254485 (2008a:47008)},
MRREVIEWER = {Jaouad Sahbani},
       DOI = {10.1007/BF02790275},
       URL = {http://dx.doi.org/10.1007/BF02790275},
}

@article {Len99,
    AUTHOR = {Lenz, D.},
     TITLE = {Random operators and crossed products},
   JOURNAL = {Math. Phys. Anal. Geom.},
  FJOURNAL = {Mathematical Physics, Analysis and Geometry. An International
              Journal Devoted to the Theory and Applications of Analysis and
              Geometry to Physics},
    VOLUME = {2},
      YEAR = {1999},
    NUMBER = {2},
     PAGES = {197--220},
      ISSN = {1385-0172},
     CODEN = {MPAGFO},
   MRCLASS = {46L55 (46L60 47B80 47N55 82B44 82D25)},
  MRNUMBER = {1733886 (2001b:46108)},
MRREVIEWER = {Justin Peters},
       DOI = {10.1023/A:1009884913829},
       URL = {http://dx.doi.org/10.1023/A:1009884913829},
}

@article {Len02,
    AUTHOR = {Lenz, D.},
     TITLE = {Singular spectrum of {L}ebesgue measure zero for
              one-dimensional quasicrystals},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {227},
      YEAR = {2002},
    NUMBER = {1},
     PAGES = {119--130},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {47B39 (39A70 47B80 47N55 81Q10 82B44)},
  MRNUMBER = {1903841 (2003k:47043)},
MRREVIEWER = {David Damanik},
       DOI = {10.1007/s002200200624},
       URL = {http://dx.doi.org/10.1007/s002200200624},
}

@article {LeSt03-Algebras,
    AUTHOR = {Lenz, D. and Stollmann, P.},
     TITLE = {Algebras of random operators associated to {D}elone dynamical
              systems},
   JOURNAL = {Math. Phys. Anal. Geom.},
  FJOURNAL = {Mathematical Physics, Analysis and Geometry. An International
              Journal Devoted to the Theory and Applications of Analysis and
              Geometry to Physics},
    VOLUME = {6},
      YEAR = {2003},
    NUMBER = {3},
     PAGES = {269--290},
      ISSN = {1385-0172},
     CODEN = {MPAGFO},
   MRCLASS = {46L60 (37B10 47B80 52C23 82B44)},
  MRNUMBER = {1997916 (2004j:46092)},
MRREVIEWER = {Fr{\'e}d{\'e}ric Klopp},
       DOI = {10.1023/A:1024900532603},
       URL = {http://dx.doi.org/10.1023/A:1024900532603},
}

@incollection {LeSt03-Delone,
    AUTHOR = {Lenz, D. and Stollmann, P.},
     TITLE = {Delone dynamical systems and associated random operators},
 BOOKTITLE = {Operator algebras and mathematical physics ({C}onstan\c ta,
              2001)},
     PAGES = {267--285},
 PUBLISHER = {Theta, Bucharest},
      YEAR = {2003},
   MRCLASS = {47B80 (37B50 46L60 52C23 82B44)},
  MRNUMBER = {2018235},
MRREVIEWER = {David Damanik},
}

@incollection {Len04,
    AUTHOR = {Lenz, D.},
     TITLE = {Singular continuous spectrum for certain quasicrystal
              {S}chr\"odinger operators},
 BOOKTITLE = {Complex analysis and dynamical systems},
    SERIES = {Contemp. Math.},
    VOLUME = {364},
     PAGES = {169--180},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2004},
   MRCLASS = {81Q10 (47A10 47B36 47N50)},
  MRNUMBER = {2099025 (2005f:81061)},
MRREVIEWER = {Jean-Michel Ghez},
       DOI = {10.1090/conm/364/06683},
       URL = {http://dx.doi.org/10.1090/conm/364/06683},
}

@article{LeSt05,
    AUTHOR = {Lenz, D. and Stollmann, P.},
     TITLE = {An ergodic theorem for {D}elone dynamical systems and
              existence of the integrated density of states},
   JOURNAL = {J. Anal. Math.},
  FJOURNAL = {Journal d'Analyse Math\'ematique},
    VOLUME = {97},
      YEAR = {2005},
     PAGES = {1--24},
      ISSN = {0021-7670},
     CODEN = {JOAMAV},
   MRCLASS = {37B10 (37A25 37N20 47B39 47B80 82B44)},
  MRNUMBER = {2274971},
MRREVIEWER = {David Damanik},
       DOI = {10.1007/BF02807400},
       URL = {http://dx.doi.org/10.1007/BF02807400},
}

@article {LePeIv07,
    AUTHOR = {Lenz, D. and Peyerimhoff, N. and Veseli{\'c}, I.},
     TITLE = {Groupoids, von {N}eumann algebras and the integrated density
              of states},
   JOURNAL = {Math. Phys. Anal. Geom.},
  FJOURNAL = {Mathematical Physics, Analysis and Geometry. An International
              Journal Devoted to the Theory and Applications of Analysis and
              Geometry to Physics},
    VOLUME = {10},
      YEAR = {2007},
    NUMBER = {1},
     PAGES = {1--41},
      ISSN = {1385-0172},
     CODEN = {MPAGFO},
   MRCLASS = {46L10 (35J10 46L51 46N55 47B80 81Q10 82B10 82B44)},
  MRNUMBER = {2340531},
MRREVIEWER = {Michael P. Lamoureux},
       DOI = {10.1007/s11040-007-9019-2},
       URL = {http://dx.doi.org/10.1007/s11040-007-9019-2},
}

@article{LeSt84,
    title = {Quasicrystals: A New Class of Ordered Structures},
   author = {Levine, D. and Steinhardt, Paul J.},
  journal = {Phys. Rev. Lett.},
   volume = {53},
    issue = {26},
    pages = {2477--2480},
     year = {1984},
    month = {Dec},
publisher = {American Physical Society},
      doi = {10.1103/PhysRevLett.53.2477},
      url = {http://link.aps.org/doi/10.1103/PhysRevLett.53.2477}
}


@article {Lig03,
    AUTHOR = {Lightwood, S. J.},
     TITLE = {Morphisms from non-periodic {$\mathbb{Z}^2$}-subshifts. {I}.
              {C}onstructing embeddings from homomorphisms},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {23},
      YEAR = {2003},
    NUMBER = {2},
     PAGES = {587--609},
      ISSN = {0143-3857},
   MRCLASS = {37B50 (37B40)},
  MRNUMBER = {1972240},
MRREVIEWER = {Anthony Quas},
       DOI = {10.1017/S014338570200130X},
       URL = {http://dx.doi.org/10.1017/S014338570200130X},
}

@incollection {Lin04,
    AUTHOR = {Lind, Douglas},
     TITLE = {Multi-dimensional symbolic dynamics},
 BOOKTITLE = {Symbolic dynamics and its applications},
    SERIES = {Proc. Sympos. Appl. Math.},
    VOLUME = {60},
     PAGES = {61--79},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2004},
   MRCLASS = {37B50 (11R09 37A05 37B10 37B40 37B45)},
  MRNUMBER = {2078846},
MRREVIEWER = {Manfred Einsiedler},
       DOI = {10.1090/psapm/060/2078846},
       URL = {http://dx.doi.org/10.1090/psapm/060/2078846},
}

@article {Lin08,
    AUTHOR = {Lindner, M.},
     TITLE = {Fredholmness and index of operators in the {W}iener algebra
              are independent of the underlying space},
   JOURNAL = {Oper. Matrices},
  FJOURNAL = {Operators and Matrices},
    VOLUME = {2},
      YEAR = {2008},
    NUMBER = {2},
     PAGES = {297--306},
      ISSN = {1846-3886},
   MRCLASS = {47A53 (46E40 47B36 47B37 47L10)},
  MRNUMBER = {2420728 (2009c:47014)},
MRREVIEWER = {Lu{\'{\i}}s P. Castro},
       DOI = {10.7153/oam-02-18},
       URL = {http://dx.doi.org/10.7153/oam-02-18},
}

@article {LiRo12,
    AUTHOR = {Lindner, M. and Roch, S.},
     TITLE = {Finite sections of random {J}acobi operators},
   JOURNAL = {SIAM J. Numer. Anal.},
  FJOURNAL = {SIAM Journal on Numerical Analysis},
    VOLUME = {50},
      YEAR = {2012},
    NUMBER = {1},
     PAGES = {287--306},
      ISSN = {0036-1429},
     CODEN = {SJNAAM},
   MRCLASS = {65J10 (47B36 60H25)},
  MRNUMBER = {2888314},
MRREVIEWER = {Peter Math{\'e}},
       DOI = {10.1137/100813877},
       URL = {http://dx.doi.org/10.1137/100813877},
}

@article {LiSe14,
    AUTHOR = {Lindner, M. and Seidel, M.},
     TITLE = {An affirmative answer to a core issue on limit operators},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {267},
      YEAR = {2014},
    NUMBER = {3},
     PAGES = {901--917},
      ISSN = {0022-1236},
   MRCLASS = {47A53 (47B07)},
  MRNUMBER = {3212726},
MRREVIEWER = {Manuel Gonz{\'a}lez},
       DOI = {10.1016/j.jfa.2014.03.002},
       URL = {http://dx.doi.org/10.1016/j.jfa.2014.03.002},
}

@article {LiTaWeWu02,
    AUTHOR = {Liu, Q.-H. and Tan, B. and Wen, Z.-X. and Wu, J.},
     TITLE = {Measure zero spectrum of a class of {S}chr\"odinger operators},
   JOURNAL = {J. Statist. Phys.},
  FJOURNAL = {Journal of Statistical Physics},
    VOLUME = {106},
      YEAR = {2002},
    NUMBER = {3-4},
     PAGES = {681--691},
      ISSN = {0022-4715},
     CODEN = {JSTPSB},
   MRCLASS = {81Q10 (47N50)},
  MRNUMBER = {1884550},
MRREVIEWER = {Jean-Michel Ghez},
       DOI = {10.1023/A:1013718624572},
       URL = {http://dx.doi.org/10.1023/A:1013718624572},
}

@article {LiQuWe14,
    AUTHOR = {Liu, Q.-H. and Qu, Y.-H. and Wen, Z.-Y.},
     TITLE = {The fractal dimensions of the spectrum of {S}turm
              {H}amiltonian},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {257},
      YEAR = {2014},
     PAGES = {285--336},
      ISSN = {0001-8708},
   MRCLASS = {28A78 (37C45 81Q10)},
  MRNUMBER = {3187651},
MRREVIEWER = {Shiah-Sen Wang},
       DOI = {10.1016/j.aim.2014.02.019},
       URL = {http://dx.doi.org/10.1016/j.aim.2014.02.019},
}

@article {LiQu15,
    AUTHOR = {Liu, Q.-H. and Qu, Y.-H.},
     TITLE = {On the {H}ausdorff dimension of the spectrum of the
              {T}hue-{M}orse {H}amiltonian},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {338},
      YEAR = {2015},
    NUMBER = {2},
     PAGES = {867--891},
      ISSN = {0010-3616},
   MRCLASS = {47A10},
  MRNUMBER = {3351061},
MRREVIEWER = {Naim L. Braha},
       DOI = {10.1007/s00220-015-2377-x},
       URL = {http://dx.doi.org/10.1007/s00220-015-2377-x},
}

@misc {LiQuYa16,
    AUTHOR = {Liu, Q.-H. and Qu, Y.-H. and Yao, X.},
     TITLE = {''{M}ixed spectral nature'' of the {T}hue-{M}orse {H}amiltonian},
      NOTE = {arXiv:1512.08011},
      YEAR = {2016},
       URL = {http://arxiv.org/abs/1512.08011},
}

@article {LuPl87,
    AUTHOR = {Lunnon, W. F. and Pleasants, P. A. B.},
     TITLE = {Quasicrystallographic tilings},
   JOURNAL = {J. Math. Pures Appl. (9)},
  FJOURNAL = {Journal de Math\'ematiques Pures et Appliqu\'ees. Neuvi\`eme
              S\'erie},
    VOLUME = {66},
      YEAR = {1987},
    NUMBER = {3},
     PAGES = {217--263},
      ISSN = {0021-7824},
     CODEN = {JMPAAM},
   MRCLASS = {52A45},
  MRNUMBER = {913854},
MRREVIEWER = {Marjorie Senechal},
}

@article {LuPl92,
    AUTHOR = {Lunnon, W. F. and Pleasants, P. A. B.},
     TITLE = {Characterization of two-distance sequences},
   JOURNAL = {J. Austral. Math. Soc. Ser. A},
  FJOURNAL = {Australian Mathematical Society. Journal. Series A. Pure
              Mathematics and Statistics},
    VOLUME = {53},
      YEAR = {1992},
    NUMBER = {2},
     PAGES = {198--218},
      ISSN = {0263-6115},
     CODEN = {JAMADS},
   MRCLASS = {11B83},
  MRNUMBER = {1175712},
MRREVIEWER = {Jacek Fabrykowski},
}

@article {Man12,
    AUTHOR = {M{\u{a}}ntoiu, M.},
     TITLE = {Rieffel's pseudodifferential calculus and spectral analysis of
              quantum {H}amiltonians},
   JOURNAL = {Ann. Inst. Fourier (Grenoble)},
  FJOURNAL = {Universit\'e de Grenoble. Annales de l'Institut Fourier},
    VOLUME = {62},
      YEAR = {2012},
    NUMBER = {4},
     PAGES = {1551--1580},
      ISSN = {0373-0956},
     CODEN = {AIFUA7},
   MRCLASS = {35S05 (46L55 47C15 81Q10)},
  MRNUMBER = {3025750},
       URL = {http://aif.cedram.org/item?id=AIF_2012__62_4_1551_0},
}

@article {Mar06,
    AUTHOR = {Martinez, C.},
     TITLE = {Spectral estimates for the one-dimensional non-self-adjoint
              {A}nderson model},
   JOURNAL = {J. Operator Theory},
  FJOURNAL = {Journal of Operator Theory},
    VOLUME = {56},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {59--88},
      ISSN = {0379-4024},
   MRCLASS = {47B80 (47A12 47B36 47N50 60H25 81Q10)},
  MRNUMBER = {2261612 (2008a:47063)},
}

@incollection {May94,
    AUTHOR = {Mayou, D.},
     NOTES = {by Hippert, F., Gratias, D.},
     TITLE = {Introduction to the theory of electronic properties of quasicrystals},
 BOOKTITLE = {Lectures on Quasicrystals},
 PUBLISHER = {Les Editions de Physique},
    ADRESS = {Les Ulis},
     PAGES = {417--462},
      ISBN = {9782868832306},
      YEAR = {1994},
}

@article {Mic51,
    AUTHOR = {Michael, E.},
     TITLE = {Topologies on spaces of subsets},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {71},
      YEAR = {1951},
     PAGES = {152--182},
      ISSN = {0002-9947},
   MRCLASS = {56.0X},
  MRNUMBER = {0042109 (13,54f)},
MRREVIEWER = {J. L. Kelley},
}

@incollection {Moo97,
    AUTHOR = {Moody, R. V.},
     TITLE = {Meyer sets and their duals},
 BOOKTITLE = {The mathematics of long-range aperiodic order ({W}aterloo,
              {ON}, 1995)},
    SERIES = {NATO Adv. Sci. Inst. Ser. C Math. Phys. Sci.},
    VOLUME = {489},
     PAGES = {403--441},
 PUBLISHER = {Kluwer Acad. Publ., Dordrecht},
      YEAR = {1997},
   MRCLASS = {52C99 (82D25)},
  MRNUMBER = {1460032},
MRREVIEWER = {Martin Henk},
}

@article {More05,
    AUTHOR = {Moreno, E.},
     TITLE = {De {B}ruijn sequences and de {B}ruijn graphs for a general
              language},
   JOURNAL = {Inform. Process. Lett.},
  FJOURNAL = {Information Processing Letters},
    VOLUME = {96},
      YEAR = {2005},
    NUMBER = {6},
     PAGES = {214--219},
      ISSN = {0020-0190},
     CODEN = {IFPLAT},
   MRCLASS = {05A05 (05C45)},
  MRNUMBER = {2179213 (2006e:05005)},
       DOI = {10.1016/j.ipl.2005.05.028},
       URL = {http://dx.doi.org/10.1016/j.ipl.2005.05.028},
}

@article {Mors21,
    AUTHOR = {Morse, H. M.},
     TITLE = {Recurrent geodesics on a surface of negative curvature},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {22},
      YEAR = {1921},
    NUMBER = {1},
     PAGES = {84--100},
      ISSN = {0002-9947},
     CODEN = {TAMTAM},
   MRCLASS = {53C22},
  MRNUMBER = {1501161},
       DOI = {10.2307/1988844},
       URL = {http://dx.doi.org/10.2307/1988844},
}

@article {MoHe38,
    AUTHOR = {Morse, M. and Hedlund, G. A.},
     TITLE = {Symbolic {D}ynamics},
   JOURNAL = {Amer. J. Math.},
  FJOURNAL = {American Journal of Mathematics},
    VOLUME = {60},
      YEAR = {1938},
    NUMBER = {4},
     PAGES = {815--866},
      ISSN = {0002-9327},
     CODEN = {AJMAAN},
   MRCLASS = {Contributed Item},
  MRNUMBER = {1507944},
       DOI = {10.2307/2371264},
       URL = {http://dx.doi.org/10.2307/2371264},
}

@article {MoHe40,
    AUTHOR = {Morse, M. and Hedlund, G. A.},
     TITLE = {Symbolic dynamics {II}. {S}turmian trajectories},
   JOURNAL = {Amer. J. Math.},
  FJOURNAL = {American Journal of Mathematics},
    VOLUME = {62},
      YEAR = {1940},
     PAGES = {1--42},
      ISSN = {0002-9327},
   MRCLASS = {70.1X},
  MRNUMBER = {0000745 (1,123d)},
MRREVIEWER = {C. B. Tompkins},
}

@article {Mos62,
    AUTHOR = {Moser, J.},
     TITLE = {On invariant curves of area-preserving mappings of an annulus},
   JOURNAL = {Nachr. Akad. Wiss. G\"ottingen Math.-Phys. Kl. II},
  FJOURNAL = {Nachrichten der Akademie der Wissenschaften in G\"ottingen.
              II. Mathematisch-Physikalische Klasse},
    VOLUME = {1962},
      YEAR = {1962},
     PAGES = {1--20},
      ISSN = {0065-5295},
   MRCLASS = {34.65 (57.48)},
  MRNUMBER = {0147741},
MRREVIEWER = {H. Ehrmann},
}

@article {NeSh98,
    AUTHOR = {Nelson, D. R. and Shnerb, N. M.},
     TITLE = {Non-{H}ermitian localization and population biology},
   JOURNAL = {Phys. Rev. E (3)},
  FJOURNAL = {Physical Review E. Statistical, Nonlinear, and Soft Matter
              Physics},
    VOLUME = {58},
      YEAR = {1998},
    NUMBER = {2, part A},
     PAGES = {1383--1403},
      ISSN = {1539-3755},
     CODEN = {PLEEE8},
   MRCLASS = {92D25 (82C31)},
  MRNUMBER = {1637117 (99g:92029)},
       DOI = {10.1103/PhysRevE.58.1383},
       URL = {http://dx.doi.org/10.1103/PhysRevE.58.1383},
}

@article {NiBe93,
    AUTHOR = {Nissen, H. U. and Beeli, C.},
     title = {ELECTRON MICROSCOPY OF QUASICRYSTALS AND THE VALIDITY OF THE TILING APPROACH},
   journal = {International Journal of Modern Physics B},
    volume = {07},
    number = {06n07},
     pages = {1387--1413},
      year = {1993},
       doi = {10.1142/S0217979293002390},
       URL = {http://www.worldscientific.com/doi/abs/10.1142/S0217979293002390},
    eprint = {http://www.worldscientific.com/doi/pdf/10.1142/S0217979293002390}
}

@misc {NiPr15,
    AUTHOR = {Nistor, V. and Prudhon, N.},
     TITLE = {Exhausting families of representations and spectra of pseudodifferential operators},
      NOTE = {arXiv:1411.7921},
      YEAR = {2015},
       URL = {http://arxiv.org/abs/1411.7921},
}

@article {OPRSS83,
    AUTHOR = {Ostlund, S. and Pandit, R. and Rand, D. and Schellnhuber, H.J. and Siggia, E.D.},
     TITLE = {One-dimensional {S}chr\"odinger equation with an almost
              periodic potential},
   JOURNAL = {Phys. Rev. Lett.},
  FJOURNAL = {Physical Review Letters},
    VOLUME = {50},
      YEAR = {1983},
    NUMBER = {23},
     PAGES = {1873--1876},
      ISSN = {0031-9007},
     CODEN = {PRLTAO},
   MRCLASS = {58F27 (81C05 82A05)},
  MRNUMBER = {702475},
MRREVIEWER = {Helmut R{\"u}ssmann},
       DOI = {10.1103/PhysRevLett.50.1873},
       URL = {http://dx.doi.org/10.1103/PhysRevLett.50.1873},
}

@article {OsKi85,
    AUTHOR = {{\"O}stlund, S. and Kim, S.-H.},
     TITLE = {Renormalization of quasiperiodic mappings},
      NOTE = {Physics of chaos and related problems (Gr{\"a}ft{\aa}vallen,
              1984)},
   JOURNAL = {Phys. Scripta},
  FJOURNAL = {Physica Scripta. An International Journal for Experimental and
              Theoretical Physics},
      YEAR = {1985},
    NUMBER = {Vol. T9},
     PAGES = {193--198},
      ISSN = {0031-8949},
   MRCLASS = {58F27 (82A25)},
  MRNUMBER = {863590},
MRREVIEWER = {W. R. Utz},
       DOI = {10.1088/0031-8949/1985/T9/031},
       URL = {http://dx.doi.org/10.1088/0031-8949/1985/T9/031},
}

@article {Pal70,
    AUTHOR = {Palais, R. S.},
     TITLE = {When proper maps are closed},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {24},
      YEAR = {1970},
     PAGES = {835--836},
      ISSN = {0002-9939},
   MRCLASS = {54.60},
  MRNUMBER = {0254818 (40 \#8025)},
MRREVIEWER = {G. S. Ungar},
}

@article {Pen79,
    AUTHOR = {Penrose, R.},
     TITLE = {Pentaplexity: a class of nonperiodic tilings of the plane},
   JOURNAL = {Math. Intelligencer},
  FJOURNAL = {The Mathematical Intelligencer},
    VOLUME = {2},
      YEAR = {1979/80},
    NUMBER = {1},
     PAGES = {32--37},
      ISSN = {0343-6993},
     CODEN = {MAINDC},
   MRCLASS = {52A45 (05B45)},
  MRNUMBER = {558670},
MRREVIEWER = {Joshua Zak},
       DOI = {10.1007/BF03024384},
       URL = {http://dx.doi.org/10.1007/BF03024384},
}

@article {Poo92,
    AUTHOR = {Poon, S. J.},
     title = {Electronic properties of quasicrystals an experimental review},
   journal = {Advances in Physics},
    volume = {41},
    number = {4},
     pages = {303--363},
      year = {1992},
       doi = {10.1080/00018739200101513},
       URL = {http://dx.doi.org/10.1080/00018739200101513},
}

@article {Pono13,
    AUTHOR = {Ponomarenko, L. A. and Gorbachev, R. V. and Yu, G. L. and Elias, D. C. and Jalil, R. and Patel, A. A. and Mishchenko, A. and Mayorov, A. S. and Woods, C. R. and Wallbank, J. R. and Mucha-Kruczynski, M. and Piot, B. A. and Potemski, M. and Grigorieva, I. V. and Novoselov, K. S. and Guinea, F. and Fal'ko, V. I. and Geim, A. K.},
     TITLE = {Cloning of Dirac fermions in graphene superlattices},
   JOURNAL = {Nature},
    VOLUME = {497},
      YEAR = {2013},
     PAGES = {594--597},
   MRCLASS = {497IS (7451SP 598EP 602PB)},
       DOI = {10.1038/nature12187},
       URL = {http://www.nature.com/nature/journal/v497/n7451/abs/nature12187.html#supplementary-information
ER},
}

@article {Prou51,
    AUTHOR = {Prouhet, M. E.},
     TITLE = {M\'{e}moire sur quelques relations entre les puissances des nombres},
   JOURNAL = {C.R. Adad. Sci. Paris},
  FJOURNAL = {Comptes Rendus des S\'{e}ances de l'Acad\'{e}mie des Sciences, Paris},
    VOLUME = {33},
    NUMBER = {1},
      YEAR = {1851},
     PAGES = {225},
}

@article {PaRi16,
    AUTHOR = {Parra, D. and Richard, S.},
     TITLE = {Continuity of the spectra for families of magnetic operators on $\mathbb{Z}^d$},
   JOURNAL = {Analysis and Mathematical Physics},
      YEAR = {2016},
     PAGES = {1--17},
      ISSN = {1664-235X},
       DOI = {10.1007/s13324-015-0121-5},
       URL = {http://dx.doi.org/10.1007/s13324-015-0121-5},
}

@article {Pei33,
    AUTHOR = {Peierls, R. E.},
     title = {Zur Theorie des Diamagnetismus von Leitungselektronen},
   journal = {Zeitschrift f{\"u}r Physik},
    volume = {80},
    number = {11},
     pages = {763--791},
      year = {1933},
      issn = {0044-3328},
       doi = {10.1007/BF01342591},
       url = {http://dx.doi.org/10.1007/BF01342591},
}

@article {Pia08,
    AUTHOR = {Piantadosi, S. T.},
     TITLE = {Symbolic dynamics on free groups},
   JOURNAL = {Discrete Contin. Dyn. Syst.},
  FJOURNAL = {Discrete and Continuous Dynamical Systems. Series A},
    VOLUME = {20},
      YEAR = {2008},
    NUMBER = {3},
     PAGES = {725--738},
      ISSN = {1078-0947},
   MRCLASS = {37B10 (11B39 37B50)},
  MRNUMBER = {2373212 (2008k:37026)},
MRREVIEWER = {Hasan Ak{\i}n},
       DOI = {10.3934/dcds.2008.20.725},
       URL = {http://dx.doi.org/10.3934/dcds.2008.20.725},
}

@article {RaWo92,
    AUTHOR = {Radin, C. and Wolff, M.},
     TITLE = {Space tilings and local isomorphism},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {42},
      YEAR = {1992},
    NUMBER = {3},
     PAGES = {355--360},
      ISSN = {0046-5755},
     CODEN = {GEMDAT},
   MRCLASS = {52C22},
  MRNUMBER = {1164542 (93c:52019)},
MRREVIEWER = {Hanna Nencka},
       DOI = {10.1007/BF02414073},
       URL = {http://dx.doi.org/10.1007/BF02414073},
}

@article {Rag10,
    AUTHOR = {Raghavan, V.},
     TITLE = {{A}l-{C}u-{F}e ({A}luminum-{C}opper-{I}ron)},
   JOURNAL = {J. Phase Equilib. Diffus.},
  FJOURNAL = {Journal of Phase Equilibria and Diffusion},
    VOLUME = {31},
      YEAR = {2010},
    NUMBER = {5},
     PAGES = {449--452},
       DOI = {10.1007/s11669-010-9743-3},
}

@article {RaBe90,
    AUTHOR = {Rammal, R. and Bellissard, J.},
     TITLE = {An algebraic semi-classical approach to {B}loch electrons in a magnetic field},
   JOURNAL = {J. Phys.},
  FJOURNAL = {Journal de Physique},
    VOLUME = {51},
      YEAR = {1990},
     PAGES = {1803--1830},
       DOI = {<10.1051/jphys:0199000510170180300},
}

@incollection {Rau83,
    AUTHOR = {Rauzy, G.},
     TITLE = {Suites \`a termes dans un alphabet fini},
 BOOKTITLE = {Seminar on number theory, 1982--1983 ({T}alence, 1982/1983)},
     PAGES = {Exp. No. 25, 16},
 PUBLISHER = {Univ. Bordeaux I, Talence},
      YEAR = {1983},
   MRCLASS = {11K31 (05A99 54H20)},
  MRNUMBER = {750326 (85j:11088)},
MRREVIEWER = {Pierre Michel},
}

@article {Ren87,
    AUTHOR = {Renault, J.},
     TITLE = {Repr\'esentation des produits crois\'es d'alg\`ebres de
              groupo\"\i des},
   JOURNAL = {J. Operator Theory},
  FJOURNAL = {Journal of Operator Theory},
    VOLUME = {18},
      YEAR = {1987},
    NUMBER = {1},
     PAGES = {67--97},
      ISSN = {0379-4024},
   MRCLASS = {46L55 (22A30 46L05)},
  MRNUMBER = {912813},
MRREVIEWER = {Elliot C. Gootman},
}

@article {Ren91,
    AUTHOR = {Renault, J.},
     TITLE = {The ideal structure of groupoid crossed product {$C^\ast$}-algebras},
      NOTE = {With an appendix by Georges Skandalis},
   JOURNAL = {J. Opera\-tor Theory},
  FJOURNAL = {Journal of Operator Theory},
    VOLUME = {25},
      YEAR = {1991},
    NUMBER = {1},
     PAGES = {3--36},
      ISSN = {0379-4024},
   MRCLASS = {46L55},
  MRNUMBER = {1191252},
MRREVIEWER = {John Quigg},
}

@article {Rie81,
    AUTHOR = {Rieffel, M. A.},
     TITLE = {{${C}^{\ast} $}-algebras associated with irrational rotations},
   JOURNAL = {Pacific J. Math.},
  FJOURNAL = {Pacific Journal of Mathematics},
    VOLUME = {93},
      YEAR = {1981},
    NUMBER = {2},
     PAGES = {415--429},
      ISSN = {0030-8730},
     CODEN = {PJMAAI},
   MRCLASS = {46L55 (46M20 58F15)},
  MRNUMBER = {623572 (83b:46087)},
MRREVIEWER = {Elliot C. Gootman},
       URL = {http://projecteuclid.org/euclid.pjm/1102736269},
}

@article {Rie89,
    AUTHOR = {Rieffel, M. A.},
     TITLE = {Continuous fields of {${C}^{\ast}$}-algebras coming from group
              cocycles and actions},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {283},
      YEAR = {1989},
    NUMBER = {4},
     PAGES = {631--643},
      ISSN = {0025-5831},
     CODEN = {MAANA},
   MRCLASS = {46L45 (22D25 46M20)},
  MRNUMBER = {990592 (90b:46120)},
MRREVIEWER = {Jeffrey Fox},
       DOI = {10.1007/BF01442857},
       URL = {http://dx.doi.org/10.1007/BF01442857},
}


@article {Rob99,
    AUTHOR = {Robinson, E. A.},
     TITLE = {On the table and the chair},
   JOURNAL = {Indag. Math. (N.S.)},
  FJOURNAL = {Koninklijke Nederlandse Akademie van Wetenschappen.
              Indagationes Mathematicae. New Series},
    VOLUME = {10},
      YEAR = {1999},
    NUMBER = {4},
     PAGES = {581--599},
      ISSN = {0019-3577},
   MRCLASS = {37B50 (05B45 05B50 52C20)},
  MRNUMBER = {1820555},
MRREVIEWER = {George E. Martin},
       DOI = {10.1016/S0019-3577(00)87911-2},
       URL = {http://dx.doi.org/10.1016/S0019-3577(00)87911-2},
}

@article {RoSi89,
    AUTHOR = {Roch, S. and Silbermann, B.},
     TITLE = {Nonstrongly converging approximation methods},
   JOURNAL = {Demonstratio Math.},
  FJOURNAL = {Demonstratio Mathematica},
    VOLUME = {22},
      YEAR = {1989},
    NUMBER = {3},
     PAGES = {651--676},
      ISSN = {0420-1213},
     CODEN = {DEMADO},
   MRCLASS = {47A50 (65J10)},
  MRNUMBER = {1041905 (91b:47026)},
MRREVIEWER = {M. Z. Nashed},
}

@article {Rud59,
    AUTHOR = {Rudin, W.},
     TITLE = {Some theorems on {F}ourier coefficients},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {10},
      YEAR = {1959},
     PAGES = {855--859},
      ISSN = {0002-9939},
   MRCLASS = {42.00},
  MRNUMBER = {0116184},
MRREVIEWER = {J.-P. Kahane},
}

@article {Sad03,
    AUTHOR = {Sadun, L.},
     TITLE = {Tiling spaces are inverse limits},
   JOURNAL = {J. Math. Phys.},
  FJOURNAL = {Journal of Mathematical Physics},
    VOLUME = {44},
      YEAR = {2003},
    NUMBER = {11},
     PAGES = {5410--5414},
      ISSN = {0022-2488},
     CODEN = {JMAPAQ},
   MRCLASS = {37B50 (52C22)},
  MRNUMBER = {2014868 (2004i:37031)},
MRREVIEWER = {Manfred Einsiedler},
       DOI = {10.1063/1.1613041},
       URL = {http://dx.doi.org/10.1063/1.1613041},
}

@incollection {Sch00,
    AUTHOR = {Schlottmann, M.},
     TITLE = {Generalized model sets and dynamical systems},
 BOOKTITLE = {Directions in mathematical quasicrystals},
    SERIES = {CRM Monogr. Ser.},
    VOLUME = {13},
     PAGES = {143--159},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2000},
   MRCLASS = {52C23 (11K70 37A05 43A25 82D25)},
  MRNUMBER = {1798991},
MRREVIEWER = {Richard Kenyon},
}

@article {Sed75,
    AUTHOR = {Seda, A. K.},
     TITLE = {A continuity property of {H}aar systems of measures},
   JOURNAL = {Ann. Soc. Sci. Bruxelles S\'er. I},
  FJOURNAL = {Annales de la Societ\'e Scientifique de Bruxelles. S\'erie I.
              Sciences Math\'ematiques, Astronomiques et Physiques},
    VOLUME = {89},
      YEAR = {1975},
    NUMBER = {4},
     PAGES = {429--433},
      ISSN = {0037-959X},
   MRCLASS = {55F10 (28A35)},
  MRNUMBER = {0402741 (53 \#6555)},
MRREVIEWER = {A. Revuz},
}

@article {Sed76,
    AUTHOR = {Seda, A. K.},
     TITLE = {Haar measures for groupoids},
   JOURNAL = {Proc. Roy. Irish Acad. Sect. A},
    VOLUME = {76},
      YEAR = {1976},
    NUMBER = {5},
     PAGES = {25--36},
   MRCLASS = {28A70 (22A99)},
  MRNUMBER = {0427598 (55 \#629)},
MRREVIEWER = {K. H. Hofmann},
}

@article {Sed86,
    AUTHOR = {Seda, A. K.},
     TITLE = {On the continuity of {H}aar measure on topological groupoids},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {96},
      YEAR = {1986},
    NUMBER = {1},
     PAGES = {115--120},
      ISSN = {0002-9939},
     CODEN = {PAMYAR},
   MRCLASS = {46L99 (22D40 28C10 43A05)},
  MRNUMBER = {813822 (87m:46146)},
MRREVIEWER = {Thierry Fack},
       DOI = {10.2307/2045664},
       URL = {http://dx.doi.org/10.2307/2045664},
}

@article {Seg47,
    AUTHOR = {Segal, I. E.},
     TITLE = {Irreducible representations of operator algebras},
   JOURNAL = {Bull. Amer. Math. Soc.},
  FJOURNAL = {Bulletin of the American Mathematical Society},
    VOLUME = {53},
      YEAR = {1947},
     PAGES = {73--88},
      ISSN = {0002-9904},
   MRCLASS = {46.0X},
  MRNUMBER = {0020217 (8,520b)},
MRREVIEWER = {A. Weil},
}

@article {SeSi12,
    AUTHOR = {Seidel, M. and Silbermann, B.},
     TITLE = {Banach algebras of operator sequences},
   JOURNAL = {Oper. Matrices},
  FJOURNAL = {Operators and Matrices},
    VOLUME = {6},
      YEAR = {2012},
    NUMBER = {3},
     PAGES = {385--432},
      ISSN = {1846-3886},
   MRCLASS = {47A58 (46H35 65J10)},
  MRNUMBER = {2987017},
MRREVIEWER = {Grzegorz Lewicki},
       DOI = {10.7153/oam-06-28},
       URL = {http://dx.doi.org/10.7153/oam-06-28},
}

@article {Sei14,
    AUTHOR = {Seidel, M.},
     TITLE = {Fredholm theory for band-dominated and related operators: a
              survey},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {445},
      YEAR = {2014},
     PAGES = {373--394},
      ISSN = {0024-3795},
   MRCLASS = {47A53 (47-02 47B07)},
  MRNUMBER = {3151282},
       DOI = {10.1016/j.laa.2013.11.048},
       URL = {http://dx.doi.org/10.1016/j.laa.2013.11.048},
}

@article{SBGC84,
    AUTHOR 	= {Shechtman, D. and Blech, I. and Gratias, D. and Cahn, J. W.},
     TITLE 	= {Metallic Phase with Long-Range Orientational Order and No Translational Symmetry},
   JOURNAL 	= {Phys. Rev. Lett.},
    VOLUME 	= {53},
      YEAR 	= {1984},
     PAGES 	= {1951--1953},             
       DOI 	= {10.1103/PhysRevLett.53.1951},
       URL 	= {http://dx.doi.org/10.1103/PhysRevLett.53.1951},
 PUBLISHER	= {American Physical Society},
 }

@article{Shu78,
    AUTHOR 	= {Shubin, M.A.},
     TITLE 	= {Almost periodic functions and partial dierential operators},
   JOURNAL 	= {Russian Math. Surv.},
    VOLUME 	= {33},
      YEAR 	= {1978},
     PAGES 	= {1--52},             
}

@article {Sie16,
    AUTHOR = {Sierpi{\'{n}}ski, W.},
     TITLE = {Sur une courbe cantorienne qui contient une image biunivoque et continue de toute courbe donn{\'{e}}e},
   JOURNAL = {C. r. hebd. Seanc. Acad. Sci. Paris},
  FJOURNAL = {Comptes Rendus de l'{A}cad{\'{e}}mie de Paris},
    VOLUME = {162},
      YEAR = {1916},
     PAGES = {629--632},
      ISSN = {0001-4036},
}

@article {SiCo12,
    AUTHOR = {Ceccherini-Silberstein, T. and Coornaert, M.},
     TITLE = {On the density of periodic configurations in strongly
              irreducible subshifts},
   JOURNAL = {Nonlinearity},
  FJOURNAL = {Nonlinearity},
    VOLUME = {25},
      YEAR = {2012},
    NUMBER = {7},
     PAGES = {2119--2131},
      ISSN = {0951-7715},
     CODEN = {NONLE5},
   MRCLASS = {37B10 (37B15 37B50)},
  MRNUMBER = {2947938},
MRREVIEWER = {Anthony Quas},
       DOI = {10.1088/0951-7715/25/7/2119},
       URL = {http://dx.doi.org/10.1088/0951-7715/25/7/2119},
}

@article {Sim82,
    AUTHOR = {Simon, B.},
     TITLE = {Almost periodic {S}chr\"odinger operators: a review},
   JOURNAL = {Adv. in Appl. Math.},
  FJOURNAL = {Advances in Applied Mathematics},
    VOLUME = {3},
      YEAR = {1982},
    NUMBER = {4},
     PAGES = {463--490},
      ISSN = {0196-8858},
   MRCLASS = {34B25 (47E05 58F11 81-02 81C05)},
  MRNUMBER = {682631},
MRREVIEWER = {Evans M. Harrell},
       DOI = {10.1016/S0196-8858(82)80018-3},
       URL = {http://dx.doi.org/10.1016/S0196-8858(82)80018-3},
}

@preamble{"\def\cprime{$'$} "}
@article {Si68,
    AUTHOR = {Simonenko, I. B.},
     TITLE = {Multidimensional discrete convolutions},
   JOURNAL = {Mat. Issled.},
  FJOURNAL = {Akademiya Nauk Moldavsko\u\i\ SSR. Institut Matematiki s
              Vychislitel\cprime nym Tsentrom. Matematicheskie
              Issledovaniya},
    VOLUME = {3},
      YEAR = {1968},
    NUMBER = {vyp. 1 (7)},
     PAGES = {108--122},
      ISSN = {0542-9994},
   MRCLASS = {46.80 (42.00)},
  MRNUMBER = {0257763 (41 \#2412)},
MRREVIEWER = {Edwin Hewitt},
}

@article {SiWi12,
    AUTHOR = {Sims, A. and Williams, D. P.},
     TITLE = {Amenability for {F}ell bundles over groupoids},
   JOURNAL = {Illinois J. Math.},
  FJOURNAL = {Illinois Journal of Mathematics},
    VOLUME = {57},
      YEAR = {2013},
    NUMBER = {2},
     PAGES = {429--444},
      ISSN = {0019-2082},
   MRCLASS = {46L55 (46L05)},
  MRNUMBER = {3263040},
MRREVIEWER = {Clifford Neves},
       URL = {http://projecteuclid.org/euclid.ijm/1408453589},
}

@article {SiMoSa89,
    AUTHOR = {Sire, Cl{\'e}ment and Mosseri, R{\'e}my and Sadoc,
              Jean-Fran{\c{c}}ois},
     TITLE = {Geometric study of a {$2$}{D} tiling related to the octagonal
              quasiperiodic tiling},
   JOURNAL = {J. Physique},
  FJOURNAL = {Le Journal de Physique},
    VOLUME = {50},
      YEAR = {1989},
    NUMBER = {24},
     PAGES = {3463--3476},
      ISSN = {0302-0738},
     CODEN = {JOPQAG},
   MRCLASS = {52C20 (05B45 11H31 52C05 82D25)},
  MRNUMBER = {1033925},
MRREVIEWER = {Hanna Nencka},
}

@article {SiMo90,
    AUTHOR = {Sire, C. and Mosseri, R.},
     TITLE = {Excitation spectrum, extended states, gap closing: some exact
              results for codimension one quasicrystals},
   JOURNAL = {J. Physique},
  FJOURNAL = {Le Journal de Physique},
    VOLUME = {51},
      YEAR = {1990},
    NUMBER = {15},
     PAGES = {1569--1583},
      ISSN = {0302-0738},
     CODEN = {JOPQAG},
   MRCLASS = {82D25},
  MRNUMBER = {1063801 (91j:82050)},
MRREVIEWER = {Eugen Belokolos},
}

@incollection {Sir94,
    AUTHOR = {Sire, C.},
     NOTES = {by Hippert, F., Gratias, D.},
     TITLE = {Properties of quasiperiodic Hamiltonians. Spectra, wavefunctions and transport},
 BOOKTITLE = {Lectures on Quasicrystals},
 PUBLISHER = {Les Editions de Physique},
    ADRESS = {Les Ulis},
     PAGES = {505--533},
      ISBN = {9782868832306},
      YEAR = {1994},
}

@article {Sol98,
    AUTHOR = {Solomyak, B.},
     TITLE = {Nonperiodicity implies unique composition for self-similar
              translationally finite tilings},
   JOURNAL = {Discrete Comput. Geom.},
  FJOURNAL = {Discrete \& Computational Geometry. An International Journal
              of Mathematics and Computer Science},
    VOLUME = {20},
      YEAR = {1998},
    NUMBER = {2},
     PAGES = {265--279},
      ISSN = {0179-5376},
     CODEN = {DCGEER},
   MRCLASS = {52C22},
  MRNUMBER = {1637896},
MRREVIEWER = {R. Blind},
       DOI = {10.1007/PL00009386},
       URL = {http://dx.doi.org/10.1007/PL00009386},
}

@article {Sta14,
    AUTHOR = {Starling, C.},
     TITLE = {Finite symmetry group actions on substitution tiling {$C^\ast$}-algebras},
   Journal = {M\"unster Journal of Mathematics},
    VOLUME = {7},
    NUMBER = {2},
     PAGES = {3814--412},
      YEAR = {2014},
       DOI = {10.17879/58269765860},
}

@article {Sut87,
    AUTHOR = {S{\"u}t{\H{o}}, A.},
     TITLE = {The spectrum of a quasiperiodic {S}chr\"odinger operator},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {111},
      YEAR = {1987},
    NUMBER = {3},
     PAGES = {409--415},
      ISSN = {0010-3616},
     CODEN = {CMPHAY},
   MRCLASS = {81C05 (47B99 82A05)},
  MRNUMBER = {900502 (88m:81032)},
MRREVIEWER = {Helge Holden},
       URL = {http://projecteuclid.org/euclid.cmp/1104159638},
}

@article {Sut89,
    AUTHOR = {S{\"u}t{\H{o}}, A.},
     TITLE = {Singular continuous spectrum on a {C}antor set of zero
              {L}ebesgue measure for the {F}ibonacci {H}amiltonian},
   JOURNAL = {J. Statist. Phys.},
  FJOURNAL = {Journal of Statistical Physics},
    VOLUME = {56},
      YEAR = {1989},
    NUMBER = {3-4},
     PAGES = {525--531},
      ISSN = {0022-4715},
     CODEN = {JSTPSB},
   MRCLASS = {82A42 (47A10 47B39 58F11 81C99 82A57)},
  MRNUMBER = {1009514 (90e:82046)},
       DOI = {10.1007/BF01044450},
       URL = {http://dx.doi.org/10.1007/BF01044450},
}

@incollection {Sut95,
    AUTHOR = {S{\"u}t{\H{o}}, A.},
     TITLE = {Schr\"odinger difference equation with deterministic ergodic
              potentials},
 BOOKTITLE = {Beyond quasicrystals ({L}es {H}ouches, 1994)},
     PAGES = {481--549},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1995},
   MRCLASS = {39A70 (28D99 81Q10 82-02 82B10)},
  MRNUMBER = {1420428},
       DOI = {10.2331/suisan.61.481},
       URL = {http://dx.doi.org/10.2331/suisan.61.481},
}

@article{TanEtAl14,
  title = {Fractal Energy Spectrum of a Polariton Gas in a Fibonacci Quasiperiodic Potential},
  author = {Tanese, D. and Gurevich, E. and Baboux, F. and Jacqmin, T. and Lema\^{\i}tre, A. and Galopin, E. and Sagnes, I. and Amo, A. and Bloch, J. and Akkermans, E.},
  journal = {Phys. Rev. Lett.},
  volume = {112},
  issue = {14},
  pages = {146404},
  numpages = {5},
  year = {2014},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.112.146404},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.112.146404}
}


@article {Tho10,
    AUTHOR = {Thomsen, K.},
     TITLE = {Semi-\'etale groupoids and applications},
   JOURNAL = {Ann. Inst. Fourier (Grenoble)},
  FJOURNAL = {Universit\'e de Grenoble. Annales de l'Institut Fourier},
    VOLUME = {60},
      YEAR = {2010},
    NUMBER = {3},
     PAGES = {759--800},
      ISSN = {0373-0956},
     CODEN = {AIFUA7},
   MRCLASS = {46L55 (37B05)},
  MRNUMBER = {2680816 (2011f:46085)},
MRREVIEWER = {Valentin Deaconu},
       URL = {http://aif.cedram.org/item?id=AIF_2010__60_3_759_0},
}

@article {Thu06,
    AUTHOR = {Thue, A.},
     TITLE = {{\"U}ber unendliche {Z}eichenreichen},
   JOURNAL = {Nor. Vidensk. Selsk. Skr. Mat. Nat.},
    VOLUME = {7},
      YEAR = {1906},
     PAGES = {1--22},
}

@article {Thu12,
    AUTHOR = {Thue, A.},
     TITLE = {{\"U}ber die gegenseitige {L}age gleicher {T}eile gewisser {Z}eichenreichen},
   JOURNAL = {Nor. Vidensk. Selsk. Skr. Mat. Nat.},
    VOLUME = {1},
      YEAR = {1912},
     PAGES = {1--67},
}

@article {Tie15,
    AUTHOR = {Tietze, H.},
     TITLE = {\"{U}ber {F}unktionen, die auf einer abgeschlossenen {M}enge
              stetig sind},
   JOURNAL = {J. Reine Angew. Math.},
  FJOURNAL = {Journal f\"ur die Reine und Angewandte Mathematik. [Crelle's
              Journal]},
    VOLUME = {145},
      YEAR = {1915},
     PAGES = {9--14},
      ISSN = {0075-4102},
   MRCLASS = {Contributed Item},
  MRNUMBER = {1580909},
       DOI = {10.1515/crll.1915.145.9},
       URL = {http://dx.doi.org/10.1515/crll.1915.145.9},
}

@article {ToTa61,
    AUTHOR = {Tomiyama, J. and Takesaki, M.},
     TITLE = {Applications of fibre bundles to the certain class of
              {${C}^{\ast} $}-algebras},
   JOURNAL = {T\^ohoku Math. J. (2)},
  FJOURNAL = {The Tohoku Mathematical Journal. Second Series},
    VOLUME = {13},
      YEAR = {1961},
     PAGES = {498--522},
      ISSN = {0040-8735},
   MRCLASS = {46.65},
  MRNUMBER = {0139025 (25 \#2465)},
MRREVIEWER = {J. M. G. Fell},
}

@article {Tom62,
    AUTHOR = {Tomiyama, J.},
     TITLE = {Topological representation of {${C}^{\ast} $}-algebras},
   JOURNAL = {T\^ohoku Math. J. (2)},
  FJOURNAL = {The Tohoku Mathematical Journal. Second Series},
    VOLUME = {14},
      YEAR = {1962},
     PAGES = {187--204},
      ISSN = {0040-8735},
   MRCLASS = {46.65},
  MRNUMBER = {0143053 (26 \#619)},
MRREVIEWER = {J. M. G. Fell},
}

@article {Tor85,
    AUTHOR = {Torpe, A. M.},
     TITLE = {{$K$}-theory for the leaf space of foliations by {R}eeb
              components},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {61},
      YEAR = {1985},
    NUMBER = {1},
     PAGES = {15--71},
      ISSN = {0022-1236},
     CODEN = {JFUAAW},
   MRCLASS = {46L80 (18F25 19K33 57R30 58G12)},
  MRNUMBER = {779738},
MRREVIEWER = {Thierry Fack},
       DOI = {10.1016/0022-1236(85)90038-2},
       URL = {http://dx.doi.org/10.1016/0022-1236(85)90038-2},
}

@article{TsInMa87,
  author={Tsai, A. P. and Inoue, A. and Masumoto, T.},
  title={A Stable Quasicrystal in {A}l-{C}u-{F}e System},
  journal={Japanese Journal of Applied Physics},
  volume={26},
  number={9A},
  pages={L1505},
  url={http://stacks.iop.org/1347-4065/26/i=9A/a=L1505},
  year={1987},
}

@article {Tyc30,
    AUTHOR = {Tychonoff, A.},
     TITLE = {\"{U}ber die topologische {E}rweiterung von {R}\"aumen},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {102},
      YEAR = {1930},
    NUMBER = {1},
     PAGES = {544--561},
      ISSN = {0025-5831},
     CODEN = {MAANA},
   MRCLASS = {Contributed Item},
  MRNUMBER = {1512595},
       DOI = {10.1007/BF01782364},
       URL = {http://dx.doi.org/10.1007/BF01782364},
}

@article {Ury24,
    AUTHOR = {Urysohn, P.},
     TITLE = {\"{U}ber die {M}etrisation der kompakten topologischen
              {R}\"aume},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {92},
      YEAR = {1924},
    NUMBER = {3-4},
     PAGES = {275--293},
      ISSN = {0025-5831},
     CODEN = {MAANA},
   MRCLASS = {Contributed Item},
  MRNUMBER = {1512215},
       DOI = {10.1007/BF01448010},
       URL = {http://dx.doi.org/10.1007/BF01448010},
}

@article {Ury25,
    AUTHOR = {Urysohn, P.},
     TITLE = {\"{U}ber die {M}\"achtigkeit der zusammenh\"angenden {M}engen},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {94},
      YEAR = {1925},
    NUMBER = {1},
     PAGES = {262--295},
      ISSN = {0025-5831},
     CODEN = {MAANA},
   MRCLASS = {Contributed Item},
  MRNUMBER = {1512258},
       DOI = {10.1007/BF01208659},
       URL = {http://dx.doi.org/10.1007/BF01208659},
}

@article {Vie22,
    AUTHOR = {Vietoris, L.},
     TITLE = {Bereiche zweiter {O}rdnung},
   JOURNAL = {Monatsh. Math. Phys.},
  FJOURNAL = {Monatshefte f\"ur Mathematik und Physik},
    VOLUME = {32},
      YEAR = {1922},
    NUMBER = {1},
     PAGES = {258--280},
      ISSN = {0026-9255},
   MRCLASS = {Contributed Item},
  MRNUMBER = {1549179},
       DOI = {10.1007/BF01696886},
       URL = {http://dx.doi.org/10.1007/BF01696886},
}

@article {Wan61,
    AUTHOR = {Wang, H.},
     TITLE = {{P}roving theorems by pattern recognition - {II}},
   JOURNAL = {Bell Syst. Tech. J.},
  FJOURNAL = {Bell System Technical Journal},
    VOLUME = {40},
      YEAR = {1961},
     ISSUE = {1},
     PAGES = {1--41},
       DOI = {10.1002/j.1538-7305.1961.tb03975.x},
}

@article {Wan37,
    AUTHOR = {Wannier, G. H.},
     TITLE = {The Structure of Electronic Excitation Levels in Insulating Crystals},
   JOURNAL = {Phys. Rev.},
  FJOURNAL = {Physical Review Letters},
    VOLUME = {52},
      YEAR = {1937},
     ISSUE = {3},
     PAGES = {191--197},
 PUBLISHER = {American Physical Society},
       DOI = {10.1103/PhysRev.52.191},
       URL = {http://link.aps.org/doi/10.1103/PhysRev.52.191},
}

@article {Wei97,
    AUTHOR = {Weidmann, J.},
     TITLE = {Strong operator convergence and spectral theory of ordinary
              differential operators},
   JOURNAL = {Univ. Iagel. Acta Math.},
  FJOURNAL = {Universitatis Iagellonicae. Acta Mathematica},
    NUMBER = {34},
      YEAR = {1997},
     PAGES = {153--163},
      ISSN = {0083-4386},
   MRCLASS = {47B25 (34L05 34L40 47A10 47E05)},
  MRNUMBER = {1458041 (98d:47053)},
MRREVIEWER = {Alexei Yu. Konstantinov},
}

@misc {Wes67,
    AUTHOR = {Westman, J. J.},
     TITLE = {Non transitive groupoid algebras},
      NOTE = {Lecture notes},
      YEAR = {1967},
      NOTE = {University of California at Irvine},      
}

@article {Wil78,
    AUTHOR = {Wilcox, C. H.},
     TITLE = {Theory of {B}loch waves},
   JOURNAL = {J. Analyse Math.},
  FJOURNAL = {Journal d'Analyse Math\'ematique},
    VOLUME = {33},
      YEAR = {1978},
     PAGES = {146--167},
      ISSN = {0021-7670},
     CODEN = {JOAMAV},
   MRCLASS = {82A60 (35P10 35Q20 42C05 78A99 81H20)},
  MRNUMBER = {516045 (82b:82068)},
MRREVIEWER = {A. H. Klotz},
       DOI = {10.1007/BF02790171},
       URL = {http://dx.doi.org/10.1007/BF02790171},
}

@misc {Wil15,
    AUTHOR = {Willet, R.},
     TITLE = {A non-amenable groupoid whose maximal and reduced ${C}^{\ast}$-algebras are the same},
      NOTE = {arXiv:1504.05615},
      YEAR = {2015},
       URL = {http://arxiv.org/abs/1504.05615},
}

@article {Yok05,
    AUTHOR = {Yokonuma, T.},
     TITLE = {Discrete sets and associated dynamical systems in a
              non-commutative setting},
   JOURNAL = {Canad. Math. Bull.},
  FJOURNAL = {Canadian Mathematical Bulletin. Bulletin Canadien de
              Math\'ematiques},
    VOLUME = {48},
      YEAR = {2005},
    NUMBER = {2},
     PAGES = {302--316},
      ISSN = {0008-4395},
     CODEN = {CMBUA3},
   MRCLASS = {37B50 (54H20)},
  MRNUMBER = {2137108},
MRREVIEWER = {Ali Messaoudi},
       DOI = {10.4153/CMB-2005-028-8},
       URL = {http://dx.doi.org/10.4153/CMB-2005-028-8},
}

@article {Zim77a,
    AUTHOR = {Zimmer, R. J.},
     TITLE = {Hyperfinite factors and amenable ergodic actions},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {41},
      YEAR = {1977},
    NUMBER = {1},
     PAGES = {23--31},
      ISSN = {0020-9910},
   MRCLASS = {46L10 (22D40 43A07)},
  MRNUMBER = {0470692 (57 \#10438)},
MRREVIEWER = {Francois Combes},
}

@article {Zim77b,
    AUTHOR = {Zimmer, R. J.},
     TITLE = {On the von {N}eumann algebra of an ergodic group action},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {66},
      YEAR = {1977},
    NUMBER = {2},
     PAGES = {289--293},
      ISSN = {0002-9939},
   MRCLASS = {28A65},
  MRNUMBER = {0460599 (57 \#592)},
MRREVIEWER = {Douglas Lind},
}

@article {Zim78,
    AUTHOR = {Zimmer, R. J.},
     TITLE = {Amenable ergodic group actions and an application to {P}oisson
              boundaries of random walks},
   JOURNAL = {J. Functional Analysis},
    VOLUME = {27},
      YEAR = {1978},
    NUMBER = {3},
     PAGES = {350--372},
   MRCLASS = {22D40 (60J50)},
  MRNUMBER = {0473096 (57 \#12775)},
MRREVIEWER = {Joel J. Westman},
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%									%
%				Book				%
%									%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@book {AnantharamanRenault00,
    AUTHOR = {Anantharaman-Delaroche, C. and Renault, J.},
     TITLE = {Amenable groupoids},
    SERIES = {Mono\-gra\-phies de L'Enseignement Math\'ematique [Monographs of
              L'Enseignement Math\'ematique]},
    VOLUME = {36},
      NOTE = {With a foreword by Georges Skandalis and Appendix B by E.
              Germain},
 PUBLISHER = {L'Enseignement Math\'e\-matique, Geneva},
      YEAR = {2000},
     PAGES = {196},
      ISBN = {2-940264-01-5},
   MRCLASS = {22A22 (22D25 43A07 46L05 46L10 46L80)},
  MRNUMBER = {1799683 (2001m:22005)},
MRREVIEWER = {Robert S. Doran},
}

@book {BaakeGrimm13,
    AUTHOR = {Baake, M. and Grimm, U.},
     TITLE = {Aperiodic order. {V}ol. 1},
    SERIES = {Encyclopedia of Mathematics and its Applications},
    VOLUME = {149},
      NOTE = {A mathematical invitation,
              With a foreword by Roger Penrose},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2013},
     PAGES = {xvi+531},
      ISBN = {978-0-521-86991-1},
   MRCLASS = {52C23 (11H06 20C35 20H15 82D25)},
  MRNUMBER = {3136260},
MRREVIEWER = {Jean-Pierre Gazeau},
       DOI = {10.1017/CBO9781139025256},
       URL = {http://dx.doi.org/10.1017/CBO9781139025256},
}

@book {BaakeMoody00,
     TITLE = {Directions in mathematical quasicrystals},
    SERIES = {CRM Monograph Series},
    VOLUME = {13},
    EDITOR = {Baake, M. and Moody, R. V.},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2000},
     PAGES = {viii+379},
      ISBN = {0-8218-2629-8},
   MRCLASS = {52C23 (52-06 82D25)},
  MRNUMBER = {1798986},
}

@book {Bol98,
    AUTHOR = {Bollob{\'a}s, B.},
     TITLE = {Modern graph theory},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {184},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {1998},
     PAGES = {xiv+394},
      ISBN = {0-387-98488-7},
   MRCLASS = {05-01 (05-02 05Cxx)},
  MRNUMBER = {1633290},
MRREVIEWER = {Jerrold W. Grossman},
       DOI = {10.1007/978-1-4612-0619-4},
       URL = {http://dx.doi.org/10.1007/978-1-4612-0619-4},
}

@book {Boncompagni57,
    AUTHOR = {Boncompagni, B.},
     TITLE = {Scritti di Leonardo Pisano matematico del secolo decimoterzo. Bd. I},
 PUBLISHER = {Tipografia delle scienze matematiche e fisiche, Rom},
      NOTE = {L'Enseignement Math\'ematique, Geneva},
      YEAR = {1857},
}

@book {CastaingValadier77,
    AUTHOR = {Castaing, C. and Valadier, M.},
     TITLE = {Convex analysis and measurable multifunctions},
    SERIES = {Lecture Notes in Mathematics, Vol. 580},
 PUBLISHER = {Springer-Verlag, Berlin-New York},
      YEAR = {1977},
     PAGES = {vii+278},
   MRCLASS = {46G99 (26A51 28A05 49A50 54C60)},
  MRNUMBER = {0467310 (57 \#7169)},
MRREVIEWER = {Vladimir L. Levin},
}

@book {CarmonaLacroix90,
    AUTHOR = {Carmona, R. and Lacroix, J.},
     TITLE = {Spectral theory of random {S}chr\"odinger operators},
    SERIES = {Probability and its Applications},
 PUBLISHER = {Birkh\"auser Boston, Inc., Boston, MA},
      YEAR = {1990},
     PAGES = {xxvi+587},
      ISBN = {0-8176-3486-X},
MRREVIEWER = {Russell A. Johnson},
       DOI = {10.1007/978-1-4612-4488-2},
       URL = {http://dx.doi.org/10.1007/978-1-4612-4488-2},
}

@book {ChandlerLindner11,
    AUTHOR = {Chandler-Wilde, S. N. and Lindner, M.},
     TITLE = {Limit operators, collective compactness, and the spectral
              theory of infinite matrices},
   JOURNAL = {Mem. Amer. Math. Soc.},
  FJOURNAL = {Memoirs of the American Mathematical Society},
    VOLUME = {210},
      YEAR = {2011},
    NUMBER = {989},
     PAGES = {viii+111},
      ISSN = {0065-9266},
     CODEN = {MAMCAU},
 PUBLISHER = {American Mathematical Society, Providence, Rhode Island},
      ISBN = {978-0-8218-5243-9},
   MRCLASS = {47-02 (47A53 47B07 47B37 47L80)},
  MRNUMBER = {2790742 (2012h:47001)},
MRREVIEWER = {Lu{\'{\i}}s P. Castro},
       DOI = {10.1090/S0065-9266-2010-00626-4},
       URL = {http://dx.doi.org/10.1090/S0065-9266-2010-00626-4},
}

@book {ChereneLouis78,
    AUTHOR = {Cherene, Jr. and Louis J.},
     TITLE = {Set valued dynamical systems and economic flow},
    SERIES = {Lecture Notes in Economics and Mathematical Systems},
    VOLUME = {158},
 PUBLISHER = {Springer-Verlag, Berlin-New York},
      YEAR = {1978},
     PAGES = {viii+83},
      ISBN = {3-540-08847-4},
   MRCLASS = {90A16},
  MRNUMBER = {506683 (80b:90031)},
MRREVIEWER = {E. Vilkas},
}

@book {Connes94,
    AUTHOR = {Connes, A.},
     TITLE = {Noncommutative geometry},
 PUBLISHER = {Academic Press, Inc., San Diego, CA},
      YEAR = {1994},
     PAGES = {xiv+661},
      ISBN = {0-12-185860-X},
   MRCLASS = {46Lxx (19K56 22D25 58B30 58G12 81T13 81V22 81V70)},
  MRNUMBER = {1303779},
MRREVIEWER = {John Roe},
}

@book {Corduneanu68,
    AUTHOR = {Corduneanu, C.},
     TITLE = {Almost periodic functions},
      NOTE = {With the collaboration of N. Gheorghiu and V. Barbu,
              Translated from the Romanian by Gitta Bernstein and Eugene
              Tomer,
              Interscience Tracts in Pure and Applied Mathematics, No. 22},
 PUBLISHER = {Interscience Publishers [John Wiley \& Sons], New
              York-London-Sydney},
      YEAR = {1968},
     PAGES = {x+237},
   MRCLASS = {42A84},
  MRNUMBER = {0481915 (58 \#2006)},
}

@book {CyconFroeseKirschSimon87,
    AUTHOR = {Cycon, H. L. and Froese, R. G. and Kirsch, W. and Simon, B.},
     TITLE = {Schr\"odinger operators with application to quantum mechanics
              and global geometry},
    SERIES = {Texts and Monographs in Physics},
   EDITION = {Study},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {1987},
     PAGES = {x+319},
      ISBN = {3-540-16758-7},
   MRCLASS = {35-02 (35J10 47F05 58G40 81C10)},
  MRNUMBER = {883643 (88g:35003)},
MRREVIEWER = {M. Demuth},
}

@book {DoranFell88,
    AUTHOR = {Doran, R. S. and Fell, J. M. G.},
     TITLE = {Representations of {${\ast}$}-algebras, locally compact groups,
              and {B}anach {${\ast}$}-algebraic bundles. {V}ol. 1},
    SERIES = {Pure and Applied Mathematics},
    VOLUME = {125},
      NOTE = {Basic representation theory of groups and algebras},
 PUBLISHER = {Academic Press, Inc., Boston, MA},
      YEAR = {1988},
     PAGES = {xviii+746},
      ISBN = {0-12-252721-6},
   MRCLASS = {46-02 (22Dxx 22Exx 46Hxx 46Lxx 46M20)},
  MRNUMBER = {936628 (90c:46001)},
MRREVIEWER = {Maurice J. Dupr{\'e}},
}

@book {Dixmier69,
    AUTHOR = {Dixmier, J.},
     TITLE = {Les {${C}^{\ast} $}-alg\`ebres et leurs repr\'esentations},
    SERIES = {Deuxi\`eme \'edition. Cahiers Scientifiques, Fasc. XXIX},
 PUBLISHER = {Gauthier-Villars \'Editeur, Paris},
      YEAR = {1969},
     PAGES = {xv+390},
   MRCLASS = {46.65},
  MRNUMBER = {0246136 (39 \#7442)},
}

@book {Dixmier77,
    AUTHOR = {Dixmier, J.},
     TITLE = {{$C\sp*$}-algebras},
      NOTE = {Translated from the French by Francis Jellett,
              North-Holland Mathematical Library, Vol. 15},
 PUBLISHER = {North-Holland Publishing Co., Amsterdam-New York-Oxford},
      YEAR = {1977},
     PAGES = {xiii+492},
      ISBN = {0-7204-0762-1},
   MRCLASS = {46L05},
  MRNUMBER = {0458185 (56 \#16388)},
}

@book {Dixmier96,
    AUTHOR = {Dixmier, J.},
     TITLE = {Les alg\`ebres d'op\'erateurs dans l'espace hilbertien
              (alg\`ebres de von {N}eumann)},
    SERIES = {Les Grands Classiques Gauthier-Villars. [Gauthier-Villars
              Great Classics]},
      NOTE = {Reprint of the second (1969) edition},
 PUBLISHER = {\'Editions Jacques Gabay, Paris},
      YEAR = {1996},
     PAGES = {x+367},
      ISBN = {2-87647-012-8},
   MRCLASS = {46Lxx (01A75 46L10)},
  MRNUMBER = {1451139 (98a:46065)},
}

@book {Dixmier81,
    AUTHOR = {Dixmier, J.},
     TITLE = {von {N}eumann algebras},
    SERIES = {North--Holland Mathematical Library},
    VOLUME = {27},
      NOTE = {With a preface by E. C. Lance,
              Translated from the second French edition by F. Jellett},
 PUBLISHER = {North--Holland Publishing Co., Amsterdam-New York},
      YEAR = {1981},
     PAGES = {xxxviii+437},
      ISBN = {0-444-86308-7},
   MRCLASS = {46-02 (16A30 22D25 46Lxx)},
  MRNUMBER = {641217 (83a:46004)},
}

@book {Elstrodt05,
    AUTHOR = {Elstrodt, J.},
     TITLE = {Ma\ss- und {I}ntegrationstheorie},
    SERIES = {Springer-Lehrbuch. [Springer Textbook]},
   EDITION = {Fourth},
      NOTE = {Grundwissen Mathematik. [Basic Knowledge in Mathematics]},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {2005},
     PAGES = {xvi+434},
      ISBN = {3-540-21390-2},
   MRCLASS = {28-01 (28-03 28Axx 28C15)},
  MRNUMBER = {2257838 (2008g:28001)},
MRREVIEWER = {Klaus Janssen},
}

@book {Fogg02,
    AUTHOR = {Fogg, N. P.},
     TITLE = {Substitutions in dynamics, arithmetics and combinatorics},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {1794},
      NOTE = {Edited by V. Berth{\'e}, S. Ferenczi, C. Mauduit and A.
              Siegel},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {2002},
     PAGES = {xviii+402},
      ISBN = {3-540-44141-7},
   MRCLASS = {37-06 (05A99 11B85 11J70 11R06 37B10 68R15)},
  MRNUMBER = {1970385 (2004c:37005)},
MRREVIEWER = {Teturo Kamae},
       DOI = {10.1007/b13861},
       URL = {http://dx.doi.org/10.1007/b13861},
}

@book {Gal83,
    AUTHOR = {Gallavotti, G.},
     TITLE = {The elements of mechanics},
    SERIES = {Texts and Monographs in Physics},
      NOTE = {Translated from the Italian},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {1983},
     PAGES = {xiv+575},
      ISBN = {0-387-11753-9},
   MRCLASS = {70-01 (58F11 58Fxx)},
  MRNUMBER = {698947},
       DOI = {10.1007/978-3-662-00731-0},
       URL = {http://dx.doi.org/10.1007/978-3-662-00731-0},
}

@book {Gromov99,
    AUTHOR = {Gromov, M.},
     TITLE = {Metric structures for {R}iemannian and non-{R}iemannian
              spaces},
    SERIES = {Progress in Mathematics},
    VOLUME = {152},
      NOTE = {Based on the 1981 French original [ MR0682063 (85e:53051)],
              With appendices by M. Katz, P. Pansu and S. Semmes,
              Translated from the French by Sean Michael Bates},
 PUBLISHER = {Birkh\"auser Boston, Inc., Boston, MA},
      YEAR = {1999},
     PAGES = {xx+585},
      ISBN = {0-8176-3898-9},
   MRCLASS = {53C23 (53-02)},
  MRNUMBER = {1699320 (2000d:53065)},
MRREVIEWER = {Igor Belegradek},
}

@book {Hausdorff14,
    AUTHOR = {Hausdorff, F.},
     TITLE = {Grundz\"uge der {M}engenlehre},
 PUBLISHER = {Reprinted 1949 by Chelsea Publishing Company, New York, N. Y.},
      YEAR = {1914},
     PAGES = {viii+476},
   MRCLASS = {27.2X},
  MRNUMBER = {0031025},
}

@book {Hausdorff62,
    AUTHOR = {Hausdorff, F.},
     TITLE = {Set theory},
    SERIES = {Second edition. Translated from the German by John R. Aumann
              et al},
 PUBLISHER = {Chelsea Publishing Co., New York},
      YEAR = {1962},
     PAGES = {352},
   MRCLASS = {04.00},
  MRNUMBER = {0141601},
}

@book {HiGr94,
    AUTHOR = {Hippert, F and Gratias, D.},
     TITLE = {Lectures on Quasicrystals},
 PUBLISHER = {Editions de Physique, Les Ulis},
      YEAR = {1994},
     PAGES = {559},
      ISBN = {9782868832306},
}

@book {HoBrTeWeSe92,
    AUTHOR = {Hoddesson, L. and Braun, E. and Teichmann, J. and Weart, S. and Seitz, F.},
     TITLE = {Out of the Crystal Maze: Chapters from the History of Solid State Physics},
 PUBLISHER = {Oxford Univ Press, New York},
      YEAR = {1992},
     PAGES = {728},
      ISBN = {978-0195053296},
}

@book {Kirsch89,
    AUTHOR = {Kirsch, W.},
     TITLE = {Random {S}chr\"odinger operators. {A} course},
 BOOKTITLE = {Schr\"odinger operators ({S}\o nderborg, 1988)},
    SERIES = {Lecture Notes in Phys.},
    VOLUME = {345},
     PAGES = {264--370},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1989},
   MRCLASS = {47F05 (35J10 35R60 81Q10 82B44)},
  MRNUMBER = {1037323},
MRREVIEWER = {Nariyuki Minami},
       DOI = {10.1007/3-540-51783-9_23},
       URL = {http://dx.doi.org/10.1007/3-540-51783-9_23},
}

@book {Kato95,
    AUTHOR = {Kato, T.},
     TITLE = {Perturbation theory for linear operators},
    SERIES = {Classics in Mathematics},
      NOTE = {Reprint of the 1980 edition},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {1995},
     PAGES = {xxii+619},
      ISBN = {3-540-58661-X},
   MRCLASS = {47A55 (46-00 47-00)},
  MRNUMBER = {1335452 (96a:47025)},
}

@book {KellendonkLenzSavinien15,
    TITLE = {Mathematics of aperiodic order},
    SERIES = {Progress in Mathematics},
    VOLUME = {309},
    EDITOR = {Kellendonk, J. and Lenz, D. and Savinien, J.},
 PUBLISHER = {Birkh\"auser/Springer, Basel},
      YEAR = {2015},
     PAGES = {xi+428},
      ISBN = {978-3-0348-0902-3; 978-3-0348-0903-0},
   MRCLASS = {52C23 (11-06 37-06)},
  MRNUMBER = {3380566},
       DOI = {10.1007/978-3-0348-0903-0},
       URL = {http://dx.doi.org/10.1007/978-3-0348-0903-0},
}

@book {Kuchment93,
    AUTHOR = {Kuchment, P.},
     TITLE = {Floquet theory for partial differential equations},
    SERIES = {Operator Theory: Advances and Applications},
    VOLUME = {60},
 PUBLISHER = {Birkh\"auser Verlag, Basel},
      YEAR = {1993},
     PAGES = {xiv+350},
      ISBN = {3-7643-2901-7},
   MRCLASS = {35-02 (35C15 35P10 47N20)},
  MRNUMBER = {1232660 (94h:35002)},
MRREVIEWER = {Yehuda Pinchover},
       DOI = {10.1007/978-3-0348-8573-7},
       URL = {http://dx.doi.org/10.1007/978-3-0348-8573-7},
}

@book {Kuratowski66,
    AUTHOR = {Kuratowski, K.},
     TITLE = {Topology. {V}ol. {I}},
    SERIES = {New edition, revised and augmented. Translated from the French
              by J. Jaworowski},
 PUBLISHER = {Academic Press, New York-London; Pa\'nstwowe Wydawnictwo
              Naukowe, Warsaw},
      YEAR = {1966},
     PAGES = {xx+560},
MRREVIEWER = {F. Burton Jones},
}

@book {Kuratowski68,
    AUTHOR = {Kuratowski, K.},
     TITLE = {Topology. {V}ol. {II}},
    SERIES = {New edition, revised and augmented. Translated from the French
              by A. Kirkor},
 PUBLISHER = {Academic Press, New York-London; Pa\'nstwowe Wydawnictwo
              Naukowe Polish Scientific Publishers, Warsaw},
      YEAR = {1968},
     PAGES = {xiv+608},
   MRCLASS = {54.00},
  MRNUMBER = {0259835 (41 \#4467)},
}

@book {Kurbatov99,
    AUTHOR = {Kurbatov, V. G.},
     TITLE = {Functional-differential operators and equations},
    SERIES = {Mathematics and its Applications},
    VOLUME = {473},
 PUBLISHER = {Kluwer Academic Publishers, Dordrecht},
      YEAR = {1999},
     PAGES = {xx+433},
      ISBN = {0-7923-5624-1},
   MRCLASS = {47G20 (34K05 34K06 46N20 47N20)},
  MRNUMBER = {1702280 (2001a:47050)},
MRREVIEWER = {Sjoerd M. Verduyn Lunel},
}

@book {LindMarcus95,
    AUTHOR = {Lind, D. and Marcus, B.},
     TITLE = {An introduction to symbolic dynamics and coding},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {1995},
     PAGES = {xvi+495},
      ISBN = {0-521-55124-2; 0-521-55900-6},
   MRCLASS = {58F03 (15A48 54H20 58F20 94A24 94B60)},
  MRNUMBER = {1369092 (97a:58050)},
MRREVIEWER = {Petr K{\.u}rka},
       DOI = {10.1017/CBO9780511626302},
       URL = {http://dx.doi.org/10.1017/CBO9780511626302},
}

@book {Lindner06,
    AUTHOR = {Lindner, M.},
     TITLE = {Infinite matrices and their finite sections},
    SERIES = {Frontiers in Mathematics},
      NOTE = {An introduction to the limit operator method},
 PUBLISHER = {Birkh\"auser Verlag, Basel},
      YEAR = {2006},
     PAGES = {xv+191},
      ISBN = {978-3-7643-7766-3; 3-7643-7766-6},
   MRCLASS = {47A50 (20F65 47A53 65J10 65R20)},
  MRNUMBER = {2253942 (2007k:47013)},
MRREVIEWER = {John Roe},
}

@book {Lothaire02,
    AUTHOR = {Lothaire, M.},
     TITLE = {Algebraic combinatorics on words},
    SERIES = {Encyclopedia of Mathematics and its Applications},
    VOLUME = {90},
      NOTE = {A collective work by Jean Berstel, Dominique Perrin, Patrice
              Seebold, Julien Cassaigne, Aldo De Luca, Steffano Varricchio,
              Alain Lascoux, Bernard Leclerc, Jean-Yves Thibon, Veronique
              Bruyere, Christiane Frougny, Filippo Mignosi, Antonio Restivo,
              Christophe Reutenauer, Dominique Foata, Guo-Niu Han, Jacques
              Desarmenien, Volker Diekert, Tero Harju, Juhani Karhumaki and
              Wojciech Plandowski,
              With a preface by Berstel and Perrin},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2002},
     PAGES = {xiv+504},
      ISBN = {0-521-81220-8},
   MRCLASS = {68R15 (05A99 05E10 20M35)},
  MRNUMBER = {1905123},
MRREVIEWER = {Patrice S{\'e}{\'e}bold},
       DOI = {10.1017/CBO9781107326019},
       URL = {http://dx.doi.org/10.1017/CBO9781107326019},
}

@book {Murphy90,
    AUTHOR = {Murphy, G. J.},
     TITLE = {{${C}^{\ast}$}-algebras and operator theory},
 PUBLISHER = {Academic Press, Inc., Boston, MA},
      YEAR = {1990},
     PAGES = {x+286},
      ISBN = {0-12-511360-9},
   MRCLASS = {46Lxx (46-01)},
  MRNUMBER = {1074574 (91m:46084)},
MRREVIEWER = {E. Gerlach},
}

@book {Loomis53,
    AUTHOR = {Loomis, L. H.},
     TITLE = {An introduction to abstract harmonic analysis},
 PUBLISHER = {D. Van Nostrand Company, Inc., Toronto-New York-London},
      YEAR = {1953},
     PAGES = {x+190},
   MRCLASS = {46.3X},
  MRNUMBER = {0054173 (14,883c)},
MRREVIEWER = {K. Yosida},
}

@book {Mey72,
    AUTHOR = {Meyer, Y.},
     TITLE = {Algebraic numbers and harmonic analysis},
      NOTE = {North-Holland Mathematical Library, Vol. 2},
 PUBLISHER = {North-Holland Publishing Co., Amsterdam-London; American
              Elsevier Publishing Co., Inc., New York},
      YEAR = {1972},
     PAGES = {x+274},
   MRCLASS = {12A15 (10F45 42A44 43A46)},
  MRNUMBER = {0485769},
MRREVIEWER = {Henri Joris},
}

@book {Naimark68,
    AUTHOR = {Naimark, M. A.},
     TITLE = {Normirovannye koltsa},
      NOTE = {Second edition, revised},
 PUBLISHER = {Izdat. ``Nauka'', Moscow},
      YEAR = {1968},
     PAGES = {664},
   MRCLASS = {46HXX (46JXX 46LXX)},
  MRNUMBER = {0355602 (50 \#8076)},
}

@book {Neumark90,
    AUTHOR = {Neumark, M. A.},
     TITLE = {Normierte {A}lgebren},
    SERIES = {Hochschulb\"ucher f\"ur Mathematik [University Books for
              Mathematics], 92},
      NOTE = {Translated from the second Russian edition by B. Mai, G.
              Tesch, R. E. Becker, M. Gebel and W. Kunze},
 PUBLISHER = {VEB Deutscher Verlag der Wissenschaften, Berlin},
      YEAR = {1990},
     PAGES = {621},
      ISBN = {3-326-00191-6},
   MRCLASS = {46-01 (46Hxx 46Jxx 46Kxx 46Lxx)},
  MRNUMBER = {1034247 (90m:46004a)},
}

@book {Palmer94,
    AUTHOR = {Palmer, T. W.},
     TITLE = {Banach algebras and the general theory of {${\ast}$}-algebras.
              {V}ol. {I}},
    SERIES = {Encyclopedia of Mathematics and its Applications},
    VOLUME = {49},
      NOTE = {Algebras and Banach algebras},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {1994},
     PAGES = {xii+794},
      ISBN = {0-521-36637-2},
   MRCLASS = {46-02 (46-01 46H05 46K05 47A99)},
  MRNUMBER = {1270014 (95c:46002)},
MRREVIEWER = {Horst Behncke},
       DOI = {10.1017/CBO9781107325777},
       URL = {http://dx.doi.org/10.1017/CBO9781107325777},
}

@book {Palmer01,
    AUTHOR = {Palmer, T. W.},
     TITLE = {Banach algebras and the general theory of {$*$}-algebras.
              {V}ol. 2},
    SERIES = {Encyclopedia of Mathematics and its Applications},
    VOLUME = {79},
      NOTE = {$*$-algebras},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2001},
     PAGES = {i--xii and 795--1617},
      ISBN = {0-521-36638-0},
   MRCLASS = {46-02 (46-01 46Kxx 46L05)},
  MRNUMBER = {1819503 (2002e:46002)},
MRREVIEWER = {Robert S. Doran},
       DOI = {10.1017/CBO9780511574757.003},
       URL = {http://dx.doi.org/10.1017/CBO9780511574757.003},
}

@book {PasturFigotin92,
    AUTHOR = {Pastur, L. and Figotin, A.},
     TITLE = {Spectra of random and almost-periodic operators},
    SERIES = {Grundlehren der Mathematischen Wissenschaften [Fundamental
              Principles of Mathematical Sciences]},
    VOLUME = {297},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {1992},
     PAGES = {viii+587},
      ISBN = {3-540-50622-5},
   MRCLASS = {47B80 (34L40 35P25 47E05 47F05 60H25 82B10 82C10)},
  MRNUMBER = {1223779 (94h:47068)},
MRREVIEWER = {Russell A. Johnson},
       DOI = {10.1007/978-3-642-74346-7},
       URL = {http://dx.doi.org/10.1007/978-3-642-74346-7},
}

@book {Petersen83,
    AUTHOR = {Petersen, K.},
     TITLE = {Ergodic theory},
    SERIES = {Cambridge Studies in Advanced Mathematics},
    VOLUME = {2},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {1983},
     PAGES = {xii+329},
      ISBN = {0-521-23632-0},
   MRCLASS = {28-02 (28D05 54H20 58F11)},
  MRNUMBER = {833286},
MRREVIEWER = {Nathaniel F. G. Martin},
       DOI = {10.1017/CBO9780511608728},
       URL = {http://dx.doi.org/10.1017/CBO9780511608728},
}

@book {ProessdorfSilbermann91,
    AUTHOR = {Pr{\"o}ssdorf, S. and Silbermann, B.},
     TITLE = {Numerical analysis for integral and related operator
              equations},
    SERIES = {Operator Theory: Advances and Applications},
    VOLUME = {52},
 PUBLISHER = {Birkh\"auser Verlag, Basel},
      YEAR = {1991},
     PAGES = {542},
      ISBN = {3-7643-2620-4},
   MRCLASS = {65R20 (45L05 47A50 47G10)},
  MRNUMBER = {1193030 (94f:65126b)},
MRREVIEWER = {Heinz W. Engl},
}

@incollection {Roch2003,
    AUTHOR = {Roch, S.},
     TITLE = {Algebras of approximation sequences: structure of fractal
              algebras},
 BOOKTITLE = {Singular integral operators, factorization and applications},
    SERIES = {Oper. Theory Adv. Appl.},
    VOLUME = {142},
     PAGES = {287--310},
 PUBLISHER = {Birkh\"auser, Basel},
      YEAR = {2003},
   MRCLASS = {47A58 (46L05 47A50 47N40)},
  MRNUMBER = {2167373 (2006f:47018)},
MRREVIEWER = {Catalin Badea},
}

@book {Sad08,
    AUTHOR = {Sadun, L.},
     TITLE = {Topology of tiling spaces},
    SERIES = {University Lecture Series},
    VOLUME = {46},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2008},
     PAGES = {x+118},
      ISBN = {978-0-8218-4727-5},
   MRCLASS = {52C22 (37B50 52C23 55N05)},
  MRNUMBER = {2446623},
MRREVIEWER = {Bernd Sing},
       DOI = {10.1090/ulect/046},
       URL = {http://dx.doi.org/10.1090/ulect/046},
}

@book {Schubert75,
    AUTHOR = {Schubert, H.},
     TITLE = {Topologie},
      NOTE = {Eine Einf{\"u}hrung,
              Vierte Auflage,
              Mathematische Leitf{\"a}den},
 PUBLISHER = {B. G. Teubner, Stuttgart},
      YEAR = {1975},
     PAGES = {328},
   MRCLASS = {54-01 (55-01)},
  MRNUMBER = {0423277 (54 \#11257)},
}

@book {Queffelec87,
    AUTHOR = {Queff{\'e}lec, M.},
     TITLE = {Substitution dynamical systems---spectral analysis},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {1294},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {1987},
     PAGES = {xiv+240},
      ISBN = {3-540-18692-1},
   MRCLASS = {54H20 (11K06 28D05 58F19)},
  MRNUMBER = {924156 (89g:54094)},
MRREVIEWER = {F. Schweiger},
}

@book {Queffelec10,
    AUTHOR = {Queff{\'e}lec, M.},
     TITLE = {Substitution dynamical systems---spectral analysis},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {1294},
   EDITION = {Second},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {2010},
     PAGES = {xvi+351},
      ISBN = {978-3-642-11211-9},
   MRCLASS = {37B10 (11K06 28D05 37A30 37A45 37B15)},
  MRNUMBER = {2590264 (2011b:37018)},
MRREVIEWER = {T{\'u}lio O. Carvalho},
       DOI = {10.1007/978-3-642-11212-6},
       URL = {http://dx.doi.org/10.1007/978-3-642-11212-6},
}

@book {Querenburg2001,
    AUTHOR = {von Querenburg, B.},
     TITLE = {Mengentheoretische {T}opologie},
   EDITION = {Third},
      NOTE = {Hochschultext. [University Text]},
 PUBLISHER = {Springer-Verlag, Berlin, New York u.a.},
      YEAR = {2001},
     PAGES = {xvi+353},
      ISBN = {3-540-67790-9},
}

@book {RabinovichRochSilbermann04,
    AUTHOR = {Rabinovich, V. and Roch, S. and Silbermann, B.},
     TITLE = {Limit operators and their applications in operator theory},
    SERIES = {Operator Theory: Advances and Applications},
    VOLUME = {150},
 PUBLISHER = {Birkh\"auser Verlag, Basel},
      YEAR = {2004},
     PAGES = {xvi+392},
      ISBN = {3-7643-7081-5},
   MRCLASS = {47-02 (35-02 35S05 47A50 47A53 47B35 47G30)},
  MRNUMBER = {2075882 (2005e:47002)},
MRREVIEWER = {Alexei Yu. Karlovich},
       DOI = {10.1007/978-3-0348-7911-8},
       URL = {http://dx.doi.org/10.1007/978-3-0348-7911-8},
}

@book {ReedSimon80,
    AUTHOR = {Reed, M. and Simon, B.},
     TITLE = {Methods of modern mathematical physics. {I}},
   EDITION = {Second},
      NOTE = {Functional analysis},
 PUBLISHER = {Academic Press, Inc. [Harcourt Brace Jovanovich, Publishers],
              New York},
      YEAR = {1980},
     PAGES = {xv+400},
      ISBN = {0-12-585050-6},
   MRCLASS = {46-01 (47-01)},
  MRNUMBER = {751959 (85e:46002)},
}

@book {Renault80,
    AUTHOR = {Renault, J.},
     TITLE = {A groupoid approach to {${C}^{\ast} $}-algebras},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {793},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1980},
     PAGES = {ii+160},
      ISBN = {3-540-09977-8},
MRREVIEWER = {A. K. Seda},
}

@book {Renault09,
    AUTHOR = {Renault, J.},
     TITLE = {{${C}^\star$}-algebras and dynamical systems},
    SERIES = {Publica\c c\~oes Matem\'aticas do IMPA. [IMPA Mathematical
              Publications]},
      NOTE = {27${^{{}}{\rm{o}}}$ Col{\'o}quio Brasileiro de
              Matem{\'a}tica. [27th Brazilian Mathematics Colloquium]},
 PUBLISHER = {Instituto Nacional de Matem\'atica Pura e Aplicada (IMPA), Rio
              de Janeiro},
      YEAR = {2009},
     PAGES = {ii+105},
      ISBN = {978-85-244-0293-7},
   MRCLASS = {46L55 (46L05)},
  MRNUMBER = {2536186 (2011e:46110)},
MRREVIEWER = {Valentin Deaconu},
}

@book {Rickart60,
    AUTHOR = {Rickart, C. E.},
     TITLE = {General theory of {B}anach algebras},
    SERIES = {The University Series in Higher Mathematics},
 PUBLISHER = {D. van Nostrand Co., Inc., Princeton, N.J.-Toronto-London-New
              York},
      YEAR = {1960},
     PAGES = {xi+394},
   MRCLASS = {46.00},
  MRNUMBER = {0115101 (22 \#5903)},
MRREVIEWER = {M. Nakamura},
}

@book {Sadun2008,
    AUTHOR = {Sadun, L.},
     TITLE = {Topology of tiling spaces},
    SERIES = {University Lecture Series},
    VOLUME = {46},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2008},
     PAGES = {x+118},
      ISBN = {978-0-8218-4727-5},
   MRCLASS = {52C22 (37B50 52C23 55N05)},
  MRNUMBER = {2446623 (2009m:52041)},
MRREVIEWER = {Bernd Sing},
       DOI = {10.1090/ulect/046},
       URL = {http://dx.doi.org/10.1090/ulect/046},
}

@book {Stollmann01,
    AUTHOR = {Stollmann, P.},
     TITLE = {Caught by disorder},
    SERIES = {Progress in Mathematical Physics},
    VOLUME = {20},
      NOTE = {Bound states in random media},
 PUBLISHER = {Birkh\"auser Boston, Inc., Boston, MA},
      YEAR = {2001},
     PAGES = {xviii+166},
      ISBN = {0-8176-4210-2},
   MRCLASS = {82B44 (81Q10 82-02)},
  MRNUMBER = {1935594 (2004a:82048)},
MRREVIEWER = {Nariyuki Minami},
       DOI = {10.1007/978-1-4612-0169-4},
       URL = {http://dx.doi.org/10.1007/978-1-4612-0169-4},
}

@book {Walters82,
    AUTHOR = {Walters, P.},
     TITLE = {An introduction to ergodic theory},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {79},
 PUBLISHER = {Springer-Verlag, New York-Berlin},
      YEAR = {1982},
     PAGES = {ix+250},
      ISBN = {0-387-90599-5},
MRREVIEWER = {M. A. Akcoglu},
}

@book {Weidmann80,
    AUTHOR = {Weidmann, J.},
     TITLE = {Linear operators in {H}ilbert spaces},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {68},
      NOTE = {Trans\-lated from the German by Joseph Sz{\"u}cs},
 PUBLISHER = {Springer-Verlag, New York-Berlin},
      YEAR = {1980},
     PAGES = {xiii+402},
      ISBN = {0-387-90427-1},
   MRCLASS = {47-01 (46-01)},
  MRNUMBER = {566954 (81e: 47001)},
}

@book {Weil40,
    AUTHOR = {Weil, A.},
     TITLE = {L'int\'egration dans les groupes topologiques et ses
              applications},
    SERIES = {Actual. Sci. Ind., no. 869},
      NOTE = {[This book has been republished by the author at Princeton, N.
              J., 1941.]},
 PUBLISHER = {Hermann et Cie., Paris},
      YEAR = {1940},
     PAGES = {158},
   MRCLASS = {20.0X},
  MRNUMBER = {0005741 (3,198b)},
MRREVIEWER = {S. Kakutani},
}

@book {Williams07,
    AUTHOR = {Williams, D. P.},
     TITLE = {Crossed products of {$C{^{\ast}}$}-algebras},
    SERIES = {Mathematical Surveys and Monographs},
    VOLUME = {134},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2007},
     PAGES = {xvi+528},
      ISBN = {978-0-8218-4242-3; 0-8218-4242-0},
   MRCLASS = {46-02 (22D25 46L05 46L35 46L55 46L85)},
  MRNUMBER = {2288954 (2007m:46003)},
MRREVIEWER = {Jonathan M. Rosenberg},
       DOI = {10.1090/surv/134},
       URL = {http://dx.doi.org/10.1090/surv/134},
}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%									%
%				Thesis				%
%									%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article {BlochThesis29,
    AUTHOR = {Bloch, F.},
     TITLE = {{\"U}ber die {Q}uantenmechanik der {E}lektronen in {K}ristallgittern},
      NOTE = {Thesis (Ph.D.)},
      TYPE = {PhD Thesis},
   JOURNAL = {Z. Phys.},
  FJOURNAL = {Zeitschrift f\"ur Physik},
    VOLUME = {52},
      YEAR = {1929},
    NUMBER = {7},
     PAGES = {555--600},
   MRCLASS = {Thesis},
      ISSN = {0044-3328},
       DOI = {10.1007/BF01339455},
       URL = {http://dx.doi.org/10.1007/BF01339455},
}

@phdthesis {DahlThesis10,
    AUTHOR = {Dahl, J. M.},
     TITLE = {The {S}pectrum of the {O}ff-diagonal {F}ibonacci {O}perator},
    SCHOOL = {Rice University (United States of America)},
      YEAR = {2010},
      TYPE = {PhD Thesis},
     PAGES = {95},
       URL = {http://gateway.proquest.com/openurl?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:dissertation&res_dat=xri:pqdiss&rft_dat=xri:pqdiss:3464152},
}

@phdthesis {GoehleThesis09,
    AUTHOR = {Goehle, G.},
     TITLE = {Groupoid crossed products},
    SCHOOL = {Dartmouth College (United States of America)},
      YEAR = {2009},
      TYPE = {PhD Thesis},
     PAGES = {327},
       URL = {http://gateway.proquest.com/openurl?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:dissertation&res_dat=xri:pqdiss&rft_dat=xri:pqdiss:3397937},
}

@phdthesis {LindnerThesis03,
    AUTHOR = {Lindner, M.},
     TITLE = {Limit Operators and Applications on the Space of Essentially Bounded Functions},
    SCHOOL = {Technische-University Chemnitz (Germany)},
      TYPE = {PhD Thesis},
      YEAR = {2003},
       URL = {http://nbn-resolving.de/urn:nbn:de:swb:ch1-200301569},
}

@phdthesis {PiantadosiThesis06,
    AUTHOR = {Piantadosi, S. T.},
     TITLE = {Symbolic dynamics on free groups},
      TYPE = {Senior Honors Thesis},
    SCHOOL = {Massachusetts Institute of Technology (United States of America)},
      YEAR = {2006},
     PAGES = {58},
       URL = {http://colala.bcs.rochester.edu/papers/thesis.pdf},
}

@phdthesis {Ramazan98,
    AUTHOR = {Ramazan, B.},
     TITLE = {Quantification par D\'{e}formation des Vari\'{e}t\'{e}s de Lie-Poisson},
    SCHOOL = {University of Orl\'{e}ans (United States of America)},
      YEAR = {1998},
      TYPE = {PhD Thesis},
}

@phdthesis {RenaultThesis78,
    AUTHOR = {Renault, J.},
     TITLE = {A {G}roupoid {A}pproach to {C}*-algebras},
    SCHOOL = {University of California, Berkeley (United States of America)},
      YEAR = {1978},
     PAGES = {221},
      TYPE = {PhD Thesis},
       URL = {http://gateway.proquest.com/openurl?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:dissertation&res_dat=xri:pqdiss&rft_dat=xri:pqdiss:7914739},
}

@phdthesis {RiethThesis95,
    AUTHOR = {Rieth, T. H.},
     TITLE = {Untersuchung der {L}okalisierung von elektronischen {E}igenzu\-st{\"a}nden in quasiperiodischen {G}ittern},
    SCHOOL = {Fakult{\"a}t f{\"u}r Naturwissenschaften der Technischen Universit{\"a}t Chemnitz-Zwickau (Germany)},
      YEAR = {1995},
     PAGES = {142},
      TYPE = {PhD Thesis},
}

@phdthesis {StarlingThesis12,
   AUTHOR = {Starling, C.},
     TITLE = {Actions of {F}inite {G}roups on {S}ubstitution {T}ilings and
              {T}heir {A}ssociated {C}*-algebras},
    SCHOOL = {University of Ottawa (Canada)},
      YEAR = {2012},
     PAGES = {182},
      TYPE = {PhD Thesis},
       URL =
              {http://gateway.proquest.com/openurl?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:dissertation&res_dat=xri:pqm&rft_dat=xri:pqdiss:NR98063},
}

@article {WannierThesis37,
    AUTHOR = {Wannier, G. H.},
     TITLE = {{T}he {S}tructure of {E}lectronic {E}xcitation {L}evels in {I}nsulating Crystals},
      NOTE = {Thesis (Ph.D.)},
   JOURNAL = {Phys. Rev.},
  FJOURNAL = {Physical Review},
    VOLUME = {52},
      YEAR = {1937},
    NUMBER = {3},
     PAGES = {191--197},
   MRCLASS = {Thesis},
       DOI = {10.1103/PhysRev.52.191 },
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%									%
%				Master				%
%									%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@MastersThesis {Sha51,
    AUTHOR = {Shapiro, H. S.},
     TITLE = {Extremal problems for polynomials and power series},
      TYPE = {Master Thesis}, 
    SCHOOL = {M.I.T., Cambridge Mass. (United States of America)},
      YEAR = {1951},
     PAGES = {74},
}

@MastersThesis {Whittaker05,
    AUTHOR = {Whittaker, M. F.},
     TITLE = {{G}roupoid ${C}^{\ast}$-{A}lgebra of the {P}inwheel {T}iling},
      TYPE = {Master Thesis},
    SCHOOL = {University of Victoria (Canada)},
      YEAR = {2005},
     PAGES = {100},
       URL = {http://dspace.library.uvic.ca/bitstream/handle/1828/776/whittaker_2005.pdf?sequence=1&isAllowed=y},
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%								   	%
%		eigene Arbeiten			   	%
%								   	%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@MastersThesis {Bec12,
    AUTHOR = {Beckus, S.},
     TITLE = {{G}eneralized {B}loch {T}heory for {Q}uasicrystals},
      TYPE = {Diploma Thesis}, 
    SCHOOL = {Friedrich-Schiller-University Jena (Germany)},
    ADRESS = {Germany},
     MONTH = {February},
     PAGES = {113},
      YEAR = {2012},
}

@article {BePo13,
    AUTHOR = {Beckus, S. and Pogorzelski, F.},
     TITLE = {Spectrum of {L}ebesgue measure zero for {J}acobi matrices of
              quasicrystals},
   JOURNAL = {Math. Phys. Anal. Geom.},
  FJOURNAL = {Mathematical Physics, Analysis and Geometry. An International
              Journal Devoted to the Theory and Applications of Analysis and
              Geometry to Physics},
    VOLUME = {16},
      YEAR = {2013},
    NUMBER = {3},
     PAGES = {289--308},
      ISSN = {1385-0172},
   MRCLASS = {81Q10 (37A30 47B80)},
  MRNUMBER = {3090833},
MRREVIEWER = {Zheng Gan},
       DOI = {10.1007/s11040-013-9131-4},
       URL = {http://dx.doi.org/10.1007/s11040-013-9131-4},
}

@article {BeLeMaCh14,
    AUTHOR = {Beckus, S. and Lenz, D. and Lindner, M. and Seifert, C.},
     TITLE = {Note on spectra of non-selfadjoint operators over dynamical systems},
   Journal = {to appear in Proceedings of the Edinburgh Mathematical Society},
      YEAR = {2016},
       URL = {http://arxiv.org/abs/1412.5926},
}

@misc {BeLeMaCh16,
    AUTHOR = {Beckus, S. and Lenz, D. and Lindner, M. and Seifert, C.},
     TITLE = {On the spectrum of operator families on discrete groups over minimal dynamical systems},
      NOTE = {arXiv:1606.08353},
      YEAR = {2016},
       URL = {http://arxiv.org/abs/1412.5926},
}

@article {BeBe16,
    AUTHOR = {Beckus, S. and Bellissard, J.},
     TITLE = {{C}ontinuity of the Spectrum of a Field of Self-Adjoint Operators},
   JOURNAL = {Annales Henri Poincar{\'e}},
  FJOURNAL = {Annales Henri Poincar\'e. A Journal of Theoretical and
              Mathematical Physics},
      YEAR = {2016},
     PAGES = {1--18},
      ISSN = {1424-0661},
       DOI = {10.1007/s00023-016-0496-3},
       URL = {http://dx.doi.org/10.1007/s00023-016-0496-3},
}

@misc {BeBeNi16,
    AUTHOR = {Beckus, S. and Bellissard, J. and de Nittis, G.},
     TITLE = {{S}pectral continuity for aperiodic quantum systems},
      NOTE = {Preprint},
      YEAR = {2016},
}

%@misc {BeBe16,
%    AUTHOR = {Beckus, S. and Bellissard, J.},
%     TITLE = {{S}pectral estimate for aperiodic quantum systems},
%      NOTE = {Preprint},
%      YEAR = {2016},
%}

